Computationally Efficient Estimation of Large Probit Models

Probit models are useful for modeling correlated discrete responses in many disciplines, including consumer choice data in economics and marketing. However, the Gaussian latent variable feature of probit models coupled with identification constraints pose significant computational challenges for its estimation and inference, especially when the dimension of the discrete response variable is large. In this paper, we propose a computationally efficient Expectation-Maximization (EM) algorithm for estimating large probit models. Our work is distinct from existing methods in two important aspects. First, instead of simulation or sampling methods, we apply and customize expectation propagation (EP), a deterministic method originally proposed for approximate Bayesian inference, to estimate moments of the truncated multivariate normal (TMVN) in the E (expectation) step. Second, we take advantage of a symmetric identification condition to transform the constrained optimization problem in the M (maximization) step into a one-dimensional problem, which is solved efficiently using Newton's method instead of off-the-shelf solvers. Our method enables the analysis of correlated choice data in the presence of more than 100 alternatives, which is a reasonable size in modern applications, such as online shopping and booking platforms, but has been difficult in practice with probit models. We apply our probit estimation method to study ordering effects in hotel search results on Expedia's online booking platform.

==> review-old.tex <==
\subsection{Related Works}
\label{sec:literature-review}
\zq{move bulk to appendix as a detailed related works section, and only retain the key references in the main text.}
In this section we review existing methods for estimating probit models. The binary probit estimation problem was studied as early as \citet{fisher1935case}. Over the years, many alternative proposals to probit estimation have been studied. Here we survey the literature according to two general approaches: frequentist methods and Bayesian methods.

\textbf{Frequentist Methods.} Most frequentist approaches center on the task of approximating
the intractable integrals associated with truncated multivariate normal densities. A prominent simulation-based approach builds on the simple idea that replaces integrals with average over samples drawn from TMVN. For example, the popular simulated maximum likelihood estimation method \citep{lerman1981use,hajivassiliou1994classical,hajivassiliou1996simulation} approximates the probit likelihood using samples drawn from TMVN: 
\begin{align*}
\int_{A_{j}} f(Z_i,X_i;\beta, \Sigma)dZ_{i} \approx \frac{1}{|L|} \sum_{\ell=1}^L f(Z_i^{(\ell)},X_i^{(\ell)};\beta, \Sigma),
\end{align*} 
where $Z_{i} =X_{i}\beta+\epsilon_{i}$ and $A_{i}$ is the appropriate truncated region of integration depending on
the probit model. The approximate log-likelihood can then maximized directly using a variety of optimization techniques including Newton-Raphson and BFGS. Simulated likelihood estimators are asymptotically equivalent to MLE when $L = \Omega(\sqrt{N})$, i.e., the number of draws from TMVN grows with the square root of the sample size. Other simulation based proposals with better theoretical properties include the method of simulated moments \citep{mcfadden1989method} and method of simulated scores \citep{hajivassiliou1998method}. In simulated moment, an approximation of the likelihood $L(\theta)$ is substituted into the objective for a moment estimator
\begin{align*}
\theta_{mm} & =\arg\min_{\theta}(d-L(\theta))^{T}W^{T}W(d-L(\theta)),
\end{align*}
 where $W$ is some given fixed distance matrix, for example derived
from the first order conditions evaluated at some fixed $\theta^{0}$,
and $d$ is an indicator of whether each alternative is chosen in
every observation. When $\theta^{0}=\theta^{\ast}$ or a consistent
estimator of $\theta^{\ast}$, this method yields an estimator that
is asymptotically equivalent to the MLE. \citet{mcfadden1989method} suggests several 
sampling methods to approximate the likelihood $L(\theta)$, and also
suggests a iterative approach where the $\theta$ in $W$ is regularly
updated by current estimates. 

To achieve efficient approximation of the likelihood, the most popular technique is the GHK sampler \citep{geweke_efficient_1991,hajivassiliou1996simulation,keane1994computationally}. The GHK sampler employs a separation of variables technique based on the Cholesky factorization of the covariance to reduce the problem to sequentially sampling from one-dimensional truncated normals. Other Monte Carlo methods such as the Gibbs sampler can also be used to draw from TMVN when approximating the likelihood. 

A popular alternative simulation-based method is the Monte Carlo EM algorithm \citep{wei1990monte,chib1998analysis,natarajan2000monte}. This
approach also employs Monte Carlo samples of TMVN, but instead of approximating the likelihood directly, it approximates the conditional expectation of the complete data log-likelihood based on current parameter estimates, which is then maximized to update the estimates. For example, \citet{natarajan2000monte} use a Gibbs
sampler that cycles through the components of the latent normal variable.
Approximating the conditional expectations in the E-step requires drawing a long chain of latent variables and then averaging over
samples drawn after some burn-in period. \citet{levine2001implementations} propose a Monte Carlo EM algorithm based on importance
sampling. Notably, they suggest recycling draws from previous iterations
 of the EM algorithm through importance sampling, in order to avoid drawing
an MC sample for each iteration of the EM algorithm. \citet{moffa2014sequential} propose another alternative to Gibbs
sampling using a sequential Monte Carlo sampling method that consists
of two stages. In the first stage samples are drawn from truncated
multivariate Student $t$-distributions, which are then updated towards
truncated multivariate normal. This allows the samples of the latent
variables to be recycled and updated from one iteration to the next
rather than re-sampled at each iteration. Other works on probit estimation, including \citet{mandt_sparse_2017} and \citet{karmakar_understanding_2021}, have also used the EM algorithm without resorting to simulations for the E step. In particular \citet{mandt_sparse_2017} also proposes to use the EP method to approximate the moments of TMVN. However, their probit model has a particular factor structure for the covariance matrix rather than using a general covariance matrix. Moreover, they do not use the symmetric trace constraint. 

\textbf{Bayesian Methods.} Bayesian analysis of probit models has been a prominent research area, since it has a natural conjugate prior. Bayesian methods for probit are often variations on the theme of iterating between
sampling latent data and estimating parameters based on posterior
distribution, often with parameter expansion and data augmentation
beyond sampling latent data to simplify the computation of posterior. For example, methods based on Gibbs sampling  \citep{mcculloch1994exact,chib1998analysis} iteratively alternate
between sampling latent variables using a Gibbs sampler and drawing
parameters from the posterior distribution. The recent work of \citet{loaiza2021scalable} uses MCMC sampling based on a symmetric prior on covariance matrices with a factor structure and achieve   scalability to larger choice sets. Their prior is constructed based on the symmetric trace constraint of \citet{burgette2012trace}. Such Bayesian methods differ from the Monte Carlo EM algorithm discussed earlier
in that after latent variables are drawn, they sample \emph{model parameters}
conditional on the latent variable using a prior on the parameters. A major challenge for the Bayesian approach to probit estimation is the selection of priors subject to identification constraints. \citet{mcculloch1994exact} ignores identification issues and uses
the inverse Wishart distribution as the prior on covariance matrix $\Sigma$,
while \cite{chib1998analysis} restricts $\Sigma$ to be a correlation
matrix, and uses a Metropolis-Hastings algorithm to sample the correlation
matrix with a uniform prior. \zq{Discuss applications of EP in Bayesian approaches to probit regression.}

Parameter expansion with data augmentation \citep{tabet2007bayesian,liu1999parameter} uses reparameterization
with data augmentation to aid in the computation of the posterior, and
requires $\Sigma$ to be a correlation matrix $R$. In the first step,
one draws the latent variable $Z$ conditional on observed variable
$Y$ and parameter $\theta=(\beta,R)$, i.e., from the TMVN,
which is achieved through Gibbs sampling from a series of univariate
truncated normals in the usual manner. In the second step, one augments
$\theta$ with $\alpha$ and draw $(\alpha,\theta)$ from the joint
posterior distribution. $\alpha$ is defined so that the expanded
model $p(Y,W\mid\theta,\alpha)$ with an appropriate prior yields
a posterior on $(\alpha,\theta)$ that is easy to compute through
another set of Gibbs sampling steps.

Works on Bayesian estimation of probit models have also studied the importance of identification conditions on the computation and statistical efficiency of the resulting estimators. For example, \citet{burgette2021symmetric} propose to address the shift invariance of multivariate probit models using the constraint that latent utilities sum to zero, instead of subtracting the latent utility of a ``reference alternative'' or ``base category'' from other coordinates. This is motivated by observations by \citet{burgette2012trace} that 
Bayesian multinomial probit predictions can be sensitive to the choice of the reference alternative, whose selection is often arbitrary and leads to an asymmetric prior. We draw inspirations from these works and use a symmetric identification constraint in the EM approach. It is worth noting that EP and close relative variational inference methods \citep{bleiVariationalInferenceReview2017} have been popular tools in Bayesian approaches to  probit estimation. However, the key difference is that in Bayesian approaches, EP is used for posterior approximation, whereas in our paper, EP is used instead for \emph{moment} approximation.

Most frequentist approaches
and Bayesian methods require efficient simulation or sampling from the truncated multivariate normal distribution. They
differ in how such samples are used. For example, direct simulation based methods such as simulated maximum likelihood use the samples to approximate the likelihood; the EM approach uses
these draws to approximate the conditional expectation of the complete data log-likelihood;
Bayesian methods use sampled draws to calculate the posteriors
of parameters. 

% It should also be noted, that \emph{drawing }samples from multidimensional
% truncated Gaussian distributions and \emph{simulating }the likelihood
% are not strictly equivalent. It is true that being able to draw samples
% enables one to simulate the likelihood, but the GHK simulator is able
% to simulate probit likelihood without explicitly drawing samples from
% the posterior. 
\textbf{What's New in Our Work.} Despite the theoretical and computational developments for probit estimation in the aforementioned works, the practical application of probit models has been limited by the significant computational challenges of simulation-based methods. In this paper, we circumvent the \emph{harder} problem of simulating or sampling from TMVN distributions by considering an alternative deterministic approach to directly approximate the moments of TMVN. Expectation propagation (EP) is proposed and developed by \citet{minkaExpectationPropagationApproximate2001a,cunningham_gaussian_2013} for truncated multivariate normal distributions. In our work, we also customize the EP approach for multinomial probit by leveraging the sparsity and involution properties of the constraint matrix, which provides further acceleration for discrete choice problems. \citet{mandt_sparse_2017} previously applied EP to estimate (multivariate) probit linear mixed models for feature selection, where the covariance matrix has a simple structure as a weighted average between the identity matrix and a linear kernel of the data matrix. In contrast, our method applies to both the multivariate and multinomial probit models, and we do not impose any constraints on the covariance matrix except for the identification constraint. We give a more detailed discussion of EP in the context of probit estimation in \cref{sec:E-step}. \zq{Namedrop a few more influential papers in the general EP area (one or two theory and some applications).}

Another innovation of our work is the use of a symmetric trace identification constraint on the precision matrix, which significantly simplifies the constrained optimization problem in the EM algorithm. This proposal is an interesting combination of ideas from Bayesian and frequentist approaches to probit estimation. \citet{burgette2012trace} proposed a symmetric trace identification constraint on the covariance matrix in a Bayesian framework. In our work, we place the constraint instead on the precision matrix, which results in considerable simplifications of the constrained optimization problem in the maximization step of our EM approach. In contrast, previous EM approaches to probit estimation often used asymmetric identification conditions, which required the use of optimization packages.

 In the absence of a natural default alternative, the choice of the reference alternative to ensure identification is somewhat arbitrary \citep{train2009discrete}. Previous works have also observed that this choice can lead to different behaviors of the estimated model. To address this issue, \citet{burgette2021symmetric} propose a symmetric identification strategy. Instead of selecting a reference item, they propose to restrict the sum of latent utilities over all alternatives to be normalized to zero. This specification leads to a rank-deficient random utility model, and \citet{burgette2021symmetric} propose a Bayesian approach with a novel prior on the space of rank-deficient covariance matrices. This approach is further studied by \citet{pan_globally_2023}. 
 See also \citet{cong2017fast}, which can be used to sample from covariance matrix restricted to planes. In our EM framework, such a symmetric identification strategy requires extending the EP algorithm to approximate rank-deficient truncated multivariate normal distributions, which we leave to future works.

% \subsection{Monte Carlo-EM Algorithms for Probit Models}

% The E-M algorithm update takes the following form for the simplified
% probit problem:
% \begin{align*}
% \Sigma^{(m+1)} & =\frac{1}{n}\sum_{i=1}^{n}\mathbb{E}\left[(Z_{i}-x_{i})(Z_{i}-x_{i})^{T}\mid Y_{i},\Sigma^{(m)}\right]
% \end{align*}
%  which requires the calculation of second moment of multi-dimensional
% truncated normal. This does not have a closed-form solution, %
% \begin{comment}
% \textbf{or do they?}
% \end{comment}
% which is why probit model estimation for covariance was challenging
% for more than 4 latent variables until Monte Carlo based EM algorithms
% were proposed. 

% \textbf{}%
% \begin{comment}
% \textbf{Another idea suggested by Imbens is to use data augmentation
% to iteratively update the conditional expectation conditional on knowing
% all but one component of $\epsilon_{i}$. This would still require
% a Gibbs sampling of $\epsilon_{i}$?}
% \end{comment}

% The Monte Carlo version of EM algorithms \cite{wei1990monte,chib1998analysis,natarajan2000monte}
% consists of approximating each posterior expectation $\mathbb{E}\left[(Z_{i}-x_{i})(Z_{i}-x_{i})^{T}\mid Y_{i},\Sigma^{(m)}\right]$
% with the average 
% \begin{align*}
% \frac{1}{n_{mc}}\sum_{\ell=1}^{n_{mc}}(Z_{i}^{(\ell)}-x_{i})(Z_{i}^{(\ell)}-x_{i})^{T}
% \end{align*}
%  where $n_{mc}$ is the total number of Monte Carlo samples, and each
% $Z_{i}^{(\ell)}$ is a draw of $Z_{i}$ from the posterior distribution
% \begin{align*}
% \mathbb{P}(Z_{i}\mid Y_{i},\Sigma^{(m)})
% \end{align*}
%  given current estimate $\Sigma^{(m)}$ and observed variable $Y_{i}$.
% Thus the heart of the matter each iteration of the MC-EM algorithm
% rests on efficiently sampling from the posterior distribution. In
% the probit models we consider in this paper, the posterior distribution
% is a multivariate truncated Gaussian. For discrete choice probit models,
% this means that if $Y_{ij}=1$, then in the region of $Z_{i}\in\mathbb{R}^{m}$
% where $Z_{ij}\geq Z_{ij'}$ for all $j'$, the distribution is proportional
% to the multivariate Gaussian $\mathcal{N}(x_{i},\Sigma^{(m)})$, whereas
% outside of this region it is zero. 

% There are a couple of approaches to drawing samples from posterior
% distributions $\mathbb{P}(Z_{i}\mid Y_{i},\Sigma^{(m)})$ conditional
% on $Y_{i}$.
% \begin{itemize}
% \item Rejection sampling is the simple approach that keeps drawing samples
% from the gaussian distribution $\mathbb{P}(Z_{i}\mid\Sigma^{(m)})$
% until the required number $n_{mc}$ of valid samples of $Z_{i}$ are
% obtained. A draw $Z_{i}^{(\ell)}$ is valid if its components are
% consist with observed value $Y_{i}$, i.e. if $Y_{ij}=1$, then $Z_{ij}^{(\ell)}\geq Z_{ij'}^{(\ell)}$
% for all $j'$. If this is not the case, the draw is rejected. Rejection
% sampling works for general distributions and not just probit, but
% it suffers two drawbacks: It may take a very long time before a valid
% sample is drawn, and the resulting approximation to $\mathbb{P}(Z_{i}\mid Y_{i},\Sigma^{(m)})$
% is a non-smooth step function. The second point is not a problem if
% we are only interested in drawing samples to approximate the posterior
% expectation, but may be a problem if we are trying to directly maximize
% the likelihood using first or second order methods, which requires
% the calculation of derivatives. In this situation, a simple solution
% suggested by McFadden is to use the logistic function to approximate
% the step function used to simulate the choice probabilities. 
% \item Importance sampling methods deal with the first drawback of rejection
% sampling that rare events take more draws to simulate. The idea of
% importance sampling is also general. Consider an integral $\int V(x)g(x)dx$
% over the density $g(x)$, which is difficult to draw from. Suppose
% however that there is another density $f(x)$ that is easy to draw
% from. We may rewrite the integral as $\int V(x)g(x)/f(x)\cdot f(x)dx$
% as long as $V(x)\neq0\Rightarrow f(x)\neq0$. To approximate the integral,
% we can then draw samples from $f(x)$, calculating $V(x)g(x)/f(x)$
% for each sample, and then averaging the results. The weight $g/f$
% is the importance of the draw from $f$. One proposal of importance
% sampling for Monte Carlo EM algorithms is that in \cite{levine2001implementations}.
% Notably, this paper suggests recycling draws from previous iterations
% of the EM algorithm through importance sampling, to avoid drawing
% an MC sample for each iteration of the EM algorithm. 
% \item We also mention the GHK simulator, which uses Cholesky factorization
% of the covariance matrix to reduce to drawing from one dimensional
% truncated normals, which can be done efficiently. However, the GHK
% simulator does not allow one to draw samples from the posterior distribution,
% but only calculates the model likelihood. \textbf{}%
% \begin{comment}
% \textbf{The GHK simulator can also be viewed as an importance sampling
% method. In light of this formulation of the GHK simulator, it is a
% problem of indepedent interest to design other importance sampling
% methods for the probit model. Discussion of GHK method here citing
% Train or Chib\&Greenberg. One drawback of the GHK simulator is that
% its formulation as given here can only simulate choice probabilities
% directly, but not efficiently draw latent samples. Finall the difference
% between simulating probability and drawing samples.}
% \end{comment}
% \item Another popular approach is through Markov Chain Monte Carlo (MCMC)
% methods, such as Gibbs sampling. To draw samples from $\mathbb{P}(Z_{i}\mid Y_{i},\Sigma^{(m)})$,
% we start with some initial $Z_{i}^{(0)}$. Starting from the first
% coordinate $Z_{i1}^{(1)}$, we draw a sample from 
% \begin{align*}
% Z_{i1}^{(1)} & \sim\mathbb{P}(Z_{i1}\mid Z_{i2}^{(0)},Z_{i3}^{(0)},\dots,Z_{im}^{(0)},Y_{i},\Sigma^{(m)})
% \end{align*}
%  which is a one dimensional distribution that is usually easier to
% draw from. In the probit case, this is a one-dimensional truncated
% normal. Now to draw the second coordinate we use 
% \begin{align*}
% Z_{i2}^{(1)} & \sim\mathbb{P}(Z_{i2}\mid Z_{i1}^{(1)},Z_{i3}^{(0)},\dots,Z_{im}^{(0)},Y_{i},\Sigma^{(m)})
% \end{align*}
%  and so on for the other coordinates of $Z_{i}^{(1)}$, always conditional
% on new draws of a coordinate as long as it is available. After we
% cycle through the coordinates of $Z_{i}^{(1)}$, we repeat the procedure
% to obtain a sequence $\{Z_{i}^{(\ell)}\}_{\ell=1}^{M}$. Under suitable
% conditions, Markov chain theory guarantees that the sequence will
% converge to the stationary distribution, i.e. the multivariate posterior
% distribution we are trying to draw from, and that two samples $Z_{i}^{\ell_{1}},Z_{i}^{\ell_{2}}$
% where $\ell_{1},\ell_{2}$ are sufficiently far from each other are
% approximately independent of each other. The last step of MCMC is
% then to select the samples $Z_{i}^{(\ell_{0})},Z_{i}^{(\ell_{0}+q)},Z_{i}^{(\ell_{0}+2q)},\dots$
% where $\ell_{0}$ is called the ``burn-in'' that guarantees approximate
% convergence, and $q$ is sufficiently large to guarantee approximate
% independence. The selected samples are then used to approximate the
% posterior expectation.
% \item A recently proposed alternative \cite{moffa2014sequential} to Gibbs
% sampling uses a sequential Monte Carlo sampling method that consists
% of two stages. In the first stage samples are drawn from truncated
% multivariate Student t-distributions, which are then updated towards
% truncated multivariate normal. This allows the samples of the latent
% variables to be recycled and updated from one iteration to the next
% rather than resampled at each iteration. 
% \item Variations on the Manski type estimators have found their way to computer
% science \cite{chen2018end}. 
% \end{itemize}
% An important issue in the Monte Carlo-based approach to approximating
% the conditional distribution is how many Monte-Carlo draws of latent
% random utilities $\epsilon_{i}$ are sufficient to yield a good estimate
% of the conditional expectation, and more importantly to ensure convergence
% of the EM algorithm. With rejection/importance sampling, this of course
% means the number of valid samples. With Markov chain methods such
% as the Gibbs sampler, this means we need to decide on how long to
% run the chain as well as the burn-in length, i.e. how many initial
% estimates will be discarded in the approximation. Most literature
% on EM algorithms for probit models only mention that this is a dataset-specific
% problem and one may need to try several heuristic rules before a suitable
% sample size/chain length can be determined. The choice of sample size
% and chain length is closely related to theoretical convergence properties
% of the Monte Carlo EM algorithm, which we will investigate in follow-up
% studies. 

==> sparsity.tex <==
\section{Sparsity Structures in Probit Models}

\subsection{Sparsity of Precision Matrix}

\subsection{Sparsity of Covariance Matrix}

\subsection{Low-rank structure of Covariance Matrix}

In general probit models, $\Sigma$ is allowed to have arbitrary correlation
patterns. However, in many problems, we may have some prior information
about the structure of $\Sigma$. For example, if $\Sigma$ represents
correlations between time periods in a panel dataset, periods that
are far apart from each other are likely to be weakly correlated,
so that $\Sigma$ is a banded matrix. In a discrete choice probit
model, we may expect the alternatives to form groups where alternatives
within the same group are substitutes/complements of one another,
whereas across groups there is little correlation between alternatives.
This corresponds to a block diagonal structure of the covariance matrix
$\Sigma$. Note that both a banded matrix and a block diagonal matrix
belong to the class of sparse matrices, so if we expect the data exhibits
sparse correlation structures, we want to exploit this information
to obtain an estimate of $\Sigma$ that is also sparse. 

The precision matrix, $\Theta=\Sigma^{-1}$, encodes information about
the conditional dependence between varaibles, and may also have sparse
structures. Since $\Theta_{jk}$ represents the conditional covariance
between $\epsilon_{ij}$ and $\epsilon_{ik}$ conditional on all the
other entries of $\epsilon_{i}$, we may expect $\Theta$ to be sparse
in a probit model of discrete choice if the maximizer is able to distinguish
between pairs of alternatives once they observe the realized latent
utilities of other alternatives.%
\begin{comment}
\textbf{Need to elaborate}
\end{comment}
{} We can also imagine a situation where the latent variables come from
some graphical model. For example, drinking coffee and lung cancer
may have high correlation, but once conditioned on smoking behavior,
they are likely to be independent from each other. In general, most
variables are somewhat marginally correlated, so sparse covariance
matrix is a rather strong requirement on independence, while sparse
precision matrix is a less stringent constraint. Thus depending on
the particular application, we are interested in solving the maximum
likelihood problem of the probit models in the setting where $\Sigma$
or $\Theta=\Sigma^{-1}$ are sparse, but we may or may not know the
support, i.e. non-zero entries, before estimation. 

In fact, we have already seen some examples that explicitly impose
such sparsity structures, for example, by requiring the covariance
matrix to have the sparse structure
\begin{align*}
\Sigma & =\begin{bmatrix}1+\rho & \rho\\
 & 1+\rho\\
 &  & 1+\rho & \rho\\
 &  &  & 1+\rho
\end{bmatrix}
\end{align*}
 both ensures identification of the model and results in a sparse
covariance estimate. Another example, also given in \cite{train2009discrete}
specifies 

\begin{align*}
\epsilon_{ij} & =-r_{i}d_{j}+\eta_{ij}
\end{align*}
 where $\eta_{ij}$ is i.i.d normal with variance $\omega$ and represents
the common component of random utility, and $r_{i}$ is normal with
variance $\sigma$ and independent of $\eta_{ij}$, and $d_{j}$ is
some indicator of group membership, with $d_{j}=1$ for $j\in J\subseteq\{1,2,3,\dots\}$,
then the covariance matrix, after relabeling, is given by 
\begin{align*}
\begin{bmatrix}\sigma B & \dots & 0 & 0\\
 & 0 & \dots & 0\\
 &  & 0 & 0\\
 &  &  & 0
\end{bmatrix}+\omega\begin{bmatrix}1\\
 & 1\\
 &  & \dots\\
 &  &  & 1
\end{bmatrix}
\end{align*}
 where $B$ is the $|J|\times|J|$ matrix with all 1s and we can check
that by specifying $\omega=1$, the model is identified. In this example,
the covariance matrix exhibits a block diagonal structure. 

However, this type of specification on the structure suffers two problems.
It requires the researcher to specify the sparsity structure, i.e.
the zero patterns and relative magnitudes of the entries before estimation.
It is also not obvious whether a particular specification leads to
an identified model.

Thus what we need is a more flexible way to incorporate our prior
knowledge about the structure of the covariance matrix: we expect
the correlation structure to be sparse, but we do not want to specify
which entries of $\Sigma$ are zero. Instead, the estimation method
encourages sparse solutions, and lets the data help us decide on an
appropriate estimate. This reasoning leads naturally to regularized
maximum likelihood estimation, where the log-likelihood is penalized
with a term that is small when the solution is sparse. We adopt this
approach and study it in detail in section 5.

Such a method is helpful for understanding the structure of the data.
For example, suppose we would like to determine the nest structure
in a nested logit model. As discussed before, nest structure is usually
pre-specified by the researcher based on outside information or domain
knowledge about the alternatives in the choice set.\textbf{ }If, however,
we are able to obtain a block diagonal estimate of $\Sigma$ in the
probit model, we would then be able to let the data inform us on how
to construct the nest. 

We also remark on the interaction between sparse structural constraints
and identification. As seen before, imposing explicit structural constraints
often reduces the degrees of freedom that sometimes leads to identification
of the unnormalized system. Encouraging sparsity in the estimate of
$\Sigma$ can be seen as implicitly reducing the degrees of freedom.
The intuition is that, even though there are multiple parameters $\Sigma$
that define the unidentified system, they are not all equivalent.
If we have some prior information about the structure of the covariance
matrix, we can select a particular model estimate based on that criterion.
This may not solve the identification problem altogether, but it should
give us a more accurate estimate of $\Sigma$ without having to specify
the exact sparsity structure before estimation. Moreover, there is
evidence that sparsity properties vary considerably among equivalent
parameters $\Sigma$ that reduce to the same $\tilde{\Sigma}$. For
example, in dimension four, we have 

\begin{align*}
\tilde{\Sigma}_{22} & =\Sigma_{22}+\Sigma_{11}-2\Sigma_{12}\\
\tilde{\Sigma}_{33} & =\Sigma_{33}+\Sigma_{11}-2\Sigma_{13}\\
\tilde{\Sigma}_{44} & =\Sigma_{44}+\Sigma_{11}-2\Sigma_{14}\\
\tilde{\Sigma}_{23} & =\Sigma_{23}+\Sigma_{11}-\Sigma_{12}-\Sigma_{13}\\
\tilde{\Sigma}_{24} & =\Sigma_{24}+\Sigma_{11}-\Sigma_{12}-\Sigma_{14}\\
\tilde{\Sigma}_{34} & =\Sigma_{34}+\Sigma_{11}-\Sigma_{13}-\Sigma_{14}
\end{align*}
 and if among the off-diagonal entries of $\Sigma$, only $\Sigma_{32}=\Sigma_{23}\neq0$,
then we can readily verify that there is no other $\Sigma'$ with
only two non-zero off-diagonal entries that also reduce to the same
$\tilde{\Sigma}$ as $\Sigma$. 

We also note that sparsity is a property of the original $\Sigma$
that is hard to preserve under many of the normalization procedures
that deal with the identification issue. For example, normalizing
with respect to a ``reference unit'', reducing $\Sigma$ to $\tilde{\Sigma}$,
does not yield a sparse matrix $\tilde{\Sigma}$, even when $\Sigma$
is sparse. The problem is that $\tilde{\Sigma}_{ij}$ all contain
$\Sigma_{11}$, hence will be non-zero in general. An exception to
this is that if there is an outside option to all the alternatives,
whose random utility has small variance (or is constant) and is uncorrelated
with that of any other alternative, $\tilde{\Sigma}$ will also be
sparse. Such an ``outside option'' is not always available. In view
of the above discussion on identification and sparsity, we take the
path that directly estimates the original covariance matrix $\Sigma$,
normalized only with respect to scale, e.g. $\beta_{1}=1$ or $\Sigma_{11}=1$,
while imposing sparsity constraints but without normalizing $\Sigma$
with respect to shifts. The hope is that asymptotically we can at
least recover one of the several $\Sigma$'s that are equivalent to
the ground truth $\Sigma^{\ast}$, such that $\Sigma$ is also sparse. 

It should be noted, however, that sparsity is a separate matter from
identification. If we adopt the normalization strategy that restricts
$\Sigma$ to be a correlation matrix, we can still apply the methods
developed in the paper to obtain sparse estimates, if we expect $\Sigma$
to have sparsity structures.

\begin{comment}
Still, because of the identification problem for unrestricted covariance
estimation, it seems that in order to impose some structural constraints
on the covariance, without specifying a particular structure \emph{a
priori} we are left with few other options. For example, reducing
in a discrete choice model, $\Sigma$ to $\tilde{\Sigma}$ often destroys
the structure of $\Sigma$, and the estimate of $\tilde{\Sigma}$
is hard to interpret. On the other hand, estimating the unidentified
system directly can lead to an estimate of $\Sigma$ that does not
exhibit the desirable structure that we want. 

Therefore, what we are after is a flexible estimation method that
can both deal with the identification problem and impose some restrictions
on the structure of the estimates, but without requiring us to stipulate
before estimation the specific structure. We accomplish this with
a \emph{model selection} approach. 
\end{comment}


\section{Sparse Covariance Estimation}
As mentioned earlier, the discussion of sparsity in probit models
is mostly limited to specifying a particular structure on the covariance
matrix, which results in fewer parameters that sometimes can also
ensure identification, for example, the specification 
\begin{align*}
\Sigma & =\begin{bmatrix}1+\rho & \rho\\
 & 1+\rho\\
 &  & 1+\rho & \rho\\
 &  &  & 1+\rho
\end{bmatrix}
\end{align*}
yields an identifiable model with a sparse covariance matrix. Such
approaches are too restrictive on the covariance matrix because it
imposes prior knowledge on the form of sparsity. Beyond these, there
have been no discussion or methods of covariance matrix estimation
with an \emph{unknown} sparse structure in probit models.

On the other hand, for Gaussian and other non-latent variable models,
sparse covariance and precision matrix estimation without prior knowledge
on zero entries has been an active area of research.

\subsection{Sparse Covariance Matrix Estimation}

On the covariance matrix side, Levina et al. \cite{levina2008sparse}
propose a LASSO-regression based method to estimate sparse covariance
matrices in settings where the variables have a natural ordering,
e.g. in time series data. Bien and Tibshirani \cite{bien2011sparse}
propose a penalized likelihood approach, where the penalization is
of the form $\|P\ast\Sigma\|_{1}$, where $P$ can be one of several
indicator matrices such as the matrix of ones, $\ast$ is elementwise
multiplication, and $\|M\|_{1}=\sum_{ij}|M_{ij}|$. This approach
is intuitive yet poses difficult optimization challenges, because
the objective is non-convex, unlike the similar problem for the precision
matrix. To circumvent this, the authors exploit the special structure
of this problem to design an MM algorithm, which is a generalized
version of EM algorithm, to iteratively alternate between finding
a convex upper bound of the penalized likelihood at the current parameter
estimate and minimizing that upper bound. 

Another important method implements the intuitive idea of thresholding
and banding to great effect.\textbf{ }The setting of such problems
are usually high-dimensional, i.e. the number of observations $n$
is smaller than the number of dimensions $m$, but the results universally
apply as long as $\frac{\log m}{n}\rightarrow0$. 

In the setting of ``bandable'' covariance matrices, Bickel and Levina
\cite{bickel2008regularized} apply the banding operator, given by
\begin{align*}
B_{k}(M) & =M_{ij}1\{|i-j|\leq k\}
\end{align*}
 and show consistency of the banded estimator with appropriate choice
of $k$ as a function of $n$ and $m$. 

In the setting of sparse covariance matrices, Bickel and Levina \cite{bickel2008covariance}
give a thresholding value $\omega_{n}\propto\sqrt{\frac{\log m}{n}}$,
and set the off-diagonal entries of the sample covariance matrix $S$
to be 0 if they do not exceed this threshold, i.e. 
\begin{align*}
\hat{\Sigma}_{ij} & =\begin{cases}
S_{ij} & \text{if }i=j\\
S_{ij}\boldsymbol{1}\{|\sigma_{ij}>\omega_{n}\} & \text{if }i\neq j
\end{cases}
\end{align*}
They show that the resulting estimator is consistent under sparsity
assumptions. An adaptive version of this method thresholds on the
correlation matrix $R=\text{diag}(\Sigma)^{-1/2}S\text{diag}(\Sigma)^{-1/2}$
to obtain $\tilde{R}$, and then scales it back to $\text{diag}(\Sigma)^{1/2}\tilde{R}\text{diag}(\Sigma)^{1/2}$,
which is equivalent to using the entry-dependent threshold $\omega_{n,ij}=\sqrt{S_{ii}S_{jj}}\omega_{n}$.

A more general approach to thresholding interpolates between shrinkage
and hard thresholding using a continuous function $h(z;\omega_{n})$:
\begin{align*}
\hat{\Sigma}_{ij} & =\begin{cases}
S_{ij} & \text{if }i=j\\
h(S_{ij};\omega_{n}) & \text{if }i\neq j
\end{cases}
\end{align*}
where $h$ satisfies the following conditions:
\begin{itemize}
\item $|h(z;\omega_{n})|\leq|z|$
\item $h(z;\omega_{n})=0$ for $|z|\leq\omega_{n}$
\item $|h(z;\omega_{n})-z|\leq\omega_{n}$
\end{itemize}
so that small values below threshold $\omega_{n}$ are set to 0, but
values above it are also (continuously) shrunken towards 0 by an amount
not larger than the threshold. This formulation is most general and
also includes hard thresholding as a special case, if we let $h(z;\omega_{n})=z\cdot1\{|z|\geq\omega_{n}\}$.
Soft thresholding takes $h(z;\omega_{n})=\text{sgn}(z)(|z|-\omega_{n})_{+}$. 

The potential usefulness of these methods for estimating sparse covariance
matrices, especially the idea of banding and thresholding, for probit
models is clear. Since all probit estimation methods are iterative,
sampling and estimation errors will likely accumulate over the iterations.
As a result, small errors could propagate and mask the underlying
sparse structure. Thresholding, if properly incorporated into the
iterations, may help filter out the true correlations from noise and
reduce accumulated errors. In practice, we observed that soft thresholding
works better than hard thresholding for probit models. This makes
sense for sparse covariance matrix, since hard thresholding tends
to concentrate relatively large errors in a few entries, so the resulting
estimate is sparse but also contains a few spurious non-zero entries. 

There is one technical problem with incorporating thresholding into
iterative algorithms for probit models. After thresholding, the resulting
matrix may not be positive definite. This is not permissible for the
probit model since we need to use that matrix as the covariance matrix
in the posterior distribution to generate new latent variables. Thus
we need to find ways to ensure that the matrix after thresholding
is positive definite. One simple idea is to select the largest $\omega_{n}$
such that the resulting matrix is positive definite. Another intuitive
idea is to find a positive definite matrix that is ``closest'' to
the thresholded correlation matrix $\hat{R}$:
\begin{align*}
\tilde{R} & =\arg\min_{A}\|\hat{R}-A\|_{F}^{2}\\
 & \text{s.t. }A\geq0,\text{diag}(A)=I_{m}
\end{align*}
 The obvious problem with this idea is again $\tilde{R}$ may not
be sparse, which can be dealt with by observing that the thresholding
method with function $h(z;\omega_{n})$ is equivalent to the following
penalized least squares formulation: 
\begin{align*}
\hat{\Sigma} & =\arg\min_{\Sigma}\frac{1}{2}\|S-\Sigma\|_{F}^{2}+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})
\end{align*}
 for appropriate $P_{\omega_{n}}$. For example, when $P_{\omega_{n}}(t)=\omega_{n}^{2}-(|t|-\omega_{n})^{2}1\{|t|<\omega_{n}\}$
corresponds to the hard thresholding method. We can then impose the
positive definite constraint directly in the penalized least squares
formulation:
\begin{align*}
\hat{\Sigma} & =\arg\min_{\lambda_{\min}(\Sigma)\geq\tau}\frac{1}{2}\|S-\Sigma\|_{F}^{2}+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})
\end{align*}
 for some $\tau>0$. The resulting problem is convex if the penalty
function is convex. See \cite{fan2016overview} for details of the
properties of this estimator. In practice, we observed that using
thresholding $h(z;\omega_{n})=\text{sgn}(z)(|z|-\omega_{n})_{+}$
with a small universal consatnt $\omega_{n}$ usually guaranteed the
positive definiteness of thresholded matrices.

\subsection{Sparse Inverse Covariance Matrix Estimation}

On the precision matrix side, there has been considerably more work
done on its sparsity than that of the covariance matrix. As mentioned
before, marginally most variables are somewhat correlated, so sparse
covariance matrices are rare. On the other hand, we can expect many
pairs of variables are conditionally independent given other variables,
resulting in sparse precision matrices. Precision matrices are also
naturally associated with graphical models. A third reason that precision
matrix regularization has been more popular is perhaps due to the
fact that the penalized MLE problem is convex in $\Theta$, given
a convex penalty, whereas the MLE problem is not convex in $\Sigma$
or $\Sigma^{-1}$. 

Similar to the covariance matrix case, there is the approach of penalized
(quasi-) maximum likelihood. When $Z_{1},\dots,Z_{n}$ are i.i.d.
$\mathcal{N}(0,\Sigma)$, the negative log-likelihood to be minimized
is 
\begin{align*}
\min_{\Theta}\text{Tr}(S\Theta)-\log\det(\Theta)
\end{align*}
where $S$ is the sample covariance and $\Theta=\Sigma^{-1}$. With
penalty on sparsity of $\Theta$, the estimate is given by 
\begin{align*}
\hat{\Theta} & =\min_{\Theta}\text{Tr}(S\Theta)-\log\det(\Theta)+\sum_{i\neq j}P_{\omega_{n}}(|\Theta_{ij}|)
\end{align*}
 where $P_{\omega_{n}}$ is some penalty to encourage sparsity of
$\Theta$. For example, a commonly used convex penality is the LASSO
penalty $P_{\omega_{n}}(t)=\omega_{n}\cdot|t|$, which has been studied,
sometimes in a different form, 
\begin{align*}
\hat{\Theta} & =\min_{\Theta}\text{Tr}(S\Theta)-\log\det(\Theta)+\|\Theta\|_{1}
\end{align*}
 in \cite{banerjee2008model,friedman2008sparse}. The approach is
known as the Graphical LASSO and is a convex problem.

Fan \cite{fan2016overview} suggests using folded convex penalties
that do not introduce bias for non-zero entries with large magnitudes,
as the LASSO penalty does. To solve the general non-convex problem
with concave penalty, the common approach is similar to that used
by \cite{bien2011sparse}, where a convex upper bounding function
is obtained through first order Taylor approximation of $P_{\omega_{n}}$,
and minimization is done on the convex surrogate. 

Another method for sparse precision matrix estimation is through column-by-column
regression. It exploits the fact that the conditional distribution
of a subset $j$ of multivariate Gaussian variables $Z\sim\mathcal{N}(0,\Sigma)$
on the rest of the set $-j$ is also a multivariate Gaussian variable:
\begin{align*}
Z_{j}\mid Z_{-j} & \sim\mathcal{N}(\alpha_{j}^{T}Z_{-j},\sigma_{j}^{2})\\
\alpha_{j} & =(\Sigma_{-j,-j})^{-1}\Sigma_{-j,j}\\
\sigma_{j}^{2} & =\Sigma_{jj}-\Sigma_{-j,j}(\Sigma_{-j,-j})^{-1}\Sigma_{-j,j}
\end{align*}
 and so we can write 
\begin{align*}
Z_{j} & =\alpha_{j}^{T}Z_{-j}+\epsilon_{j}\\
\epsilon_{j} & \sim\mathcal{N}(0,\sigma_{j}^{2})
\end{align*}
 Moreover, matrix inversion implies 
\begin{align*}
\Theta_{jj} & =\sigma_{j}^{-2}\\
\Theta_{-j,j} & =-\sigma_{j}^{-2}\alpha_{j}
\end{align*}
 so that we can recover $\Theta$ column-by-column by regressing $Z_{j}$
on $Z_{-j}$, i.e. by regressing each column of the data matrix $Z_{ij}\in\mathbb{R}^{n\times m}$
on the rest of the columns, for example using LASSO regression to
encourage sparsity on $\alpha_{j}$. In \cite{athey2019ensemble},
the authors also employ this regression method in the context of estimating
counterfactuals in panel data, where this method is referred to as
the ``horizontal regression'' method. The formulae above are also
useful for our later discussion of Gibbs sampling of latent variables
in probit models, where each entry of the latent vector is drawn according
to the Gaussian distribution above, truncated conditional on observed
choice data. This allows us to propose a sparse precision matrix estimation
in probit models using an Monte Carlo EM algorithm with Gibbs sampling,
where sampling and estimation are done directly using the precision
matrix instead of covariance matrix, to reduce simulation and computation
inaccuracies. 

\begin{comment}
Use this method combined with MCMC methods to do sparse precision
matrix estimation.

1. Generate latent variables as usual and then do horizontal regression.

2. Directly use precision matrix in Gibbs sampling step: $Z_{ij}\mid Z_{-ij}\sim\mathcal{N}(\alpha_{j}^{T}Z_{-j},\sigma_{j}^{2})$
with parameters uniquely determined from the $j$-th column of $\Theta$,
and $Z_{ij}$ is truncated of course.
\end{comment}

\section{Estimation of Probit Models with Sparsity Structures}
In this section, we finally turn to the maximum likelihood estimation
problem of the unidentified probit model, where we would like to obtain
estimates that exhibit certain sparsity structures. As a reminder,
the intuition behind our method is that the equivalent parameters
$\Sigma$ that define the unidentified probit model are not all the
same. By selecting the ones that conform to our sparsity requirements,
we can circumvent the identification problem and satisfy the sparsity
requirement at the same time. We first review the EM algorithm, then
present sparsity regularized maximum likelihood estimation problem
for probit models, before going into the details of how to solve them
with modified versions of Monte Carlo EM algorithms. 

\subsection{Penalty Regularized Sparse Covariance/Precision Matrix Estimation
in Probit Models}

Now we turn to the problem of estimating $\Sigma$ when $\Sigma$
or $\Theta=\Sigma^{-1}$ are sparse in probit models. We propose several
approaches to estimating sparse structures in probit models, which
rely on combining the MC-EM algorithms for probit models with unstructured
covariance matrices, and the penalized maximum likelihood and penalized
regression methods discussed in the previous section.

Recall the log-likelihood of the unidentified probit model is given
by 
\begin{align*}
\log L(X,Y\mid\theta,\Sigma) & =\sum_{i}\log\int_{A_{i}}f(Z_{i}\mid X_{i},\beta,\Sigma)dZ_{i1}\dots dZ_{im}\\
 & =-\frac{n}{2}\log\det(\Sigma)+\sum_{i}\log\int_{A_{i}}\exp(-\frac{1}{2}(Z_{i}-X_{i}\beta)^{T}\Sigma^{-1}(Z_{i}-X_{i}\beta))dZ_{i}
\end{align*}
 where the latent variable $Z_{i}\sim\mathcal{N}(X_{i}\beta,\Sigma)$,
and $A_{i}$ is the region corresponding to the specification of $Y_{i}$,
the observed variable, given $Z_{i}$. We propose to modify the log-likelihood
with a penalty term 
\begin{align}
\max_{\beta,\Sigma}\log L(X,Y\mid\beta,\Sigma)-P(\Sigma)
\end{align}
 that encourages certain structural characteristics of the covariance
matrix $\Sigma$ or inverse covariance matrix $\Sigma^{-1}$. For
example, $P$ is small when $\Sigma$ is sparse. This model selection
approach to estimation has had a wide impact on statistics, starting
with the LASSO estimator of Tibshirani \cite{tibshirani1996regression}.
Here, instead of being used to select covariates most relevant for
a prediction task, model selection is applied to the covariance matrix
to select a sparse estimate, at the same time circumventing identification
problems. Note that normalization with respect to scale is still necessary,
but this can be done by setting a component of $\beta$ or $\Sigma$
to 1. 

To solve the penalized MLE problem, we need to specify the exact form
of $P$. The following choices of convex sparsity penalties have been
used in regression settings:
\begin{itemize}
\item $P(\Sigma)=\lambda_{n}\cdot\sum_{i\neq j}|\Sigma_{ij}|$ (Bien and
Tibshirani \cite{bien2011sparse})
\item $P(\Sigma)=\lambda_{n}\cdot\sum_{i\neq j}|(\Sigma^{-1})_{ij}|$ (Freedman,
Hastie, and Tibshirani\cite{friedman2008sparse})
\end{itemize}
These penalties look similar, but are quite different in terms of
the associated optimization problems. As we will see, the one with
$\Sigma^{-1}$ is much easier to solve using EM algorithms, as the
maximization step involves a convex optimization problem, which is
not the case for the first penalty. 

Not all sparse estimations are written in the form of penalized maximum
likelihood. Recall that for sparse covariance matrix estimation using
banding and thresholding, the problem can be written as penalized
least squares
\begin{align*}
\hat{\Sigma} & =\arg\min_{\Sigma}\frac{1}{2}\|S-\Sigma\|_{F}^{2}+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})
\end{align*}
 where $S$ is the sample covariance matrix, and $P_{\omega_{n}}$
are penalty functions corresponding to banding or hard/soft thresholding.
Similarly, the column-by-column regression method corresponds to the
following LASSO regression
\begin{align*}
\arg\min_{\alpha_{j}\in\mathbb{R}^{m-1}}\frac{1}{2n}\sum_{i}|Z_{ij}-Z_{i(-j)}\alpha_{j}|^{2}+\lambda_{j}\|\alpha_{j}\|_{1}
\end{align*}

In latent variable models, since we do not observe the latent variables
$Z_{i}$ and $S$, the natural idea is to replace the objectives with
the conditional versions given observed variables $Y_{i}$, resulting
in 
\begin{align}
\hat{\Sigma} & =\arg\min_{\Sigma}\frac{1}{2}\mathbb{E}\left[\|S-\Sigma\|_{F}^{2}\mid X,Y,\Sigma\right]+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})
\end{align}
 and 
\begin{align*}
\arg\min_{\alpha_{j}\in\mathbb{R}^{m-1}}\frac{1}{2n}\sum_{i}\mathbb{E}\left[|Z_{ij}-Z_{i(-j)}\alpha_{j}|^{2}\mid X,Y,\Sigma\right]+\lambda_{j}\|\alpha_{j}\|_{1}
\end{align*}

These optimization problems are non-convex and complicated, but their
E-M versions are considerably simplified, with corresponding algorithms
being direct generalizations of the non-latent counterparts. In what
follows, we develop algorithms associated with the penalized maximum
likelihood or penalized regression problems for the probit model.
For the sparse covariance matrix estimation problem, we focus on using
the banding and thresholding methods in iterations of MC-EM algorithms,
as the covariance LASSO problem is challenging in terms of optimization.
For the sparse precision matrix estimation problem, we investigate
the graphical LASSO approach, and the column-by-column (or horizontal)
regression approach, both combined with the MC-EM algorithms for probit
models. 

\begin{comment}
, as well as describe the algorithms used to carry out the optimization
procedure. For the sparse covariance matrix estimation problem, we
focus on using the banding and thresholding methods in iterations
of MC-EM algorithms. For the sparse precision matrix estimation problem,
we investigate two sparsity methods, namely the Graphical LASSO approach,
and the column-by-column (or horizontal) regression approach, both
combined with the MC-EM algorithms for probit models. 

Similarly, penalizing the negative (quasi) log-likelihood $\text{Tr}(S\Theta)-\log\det(\Theta)$
with 

\begin{align*}
\text{Tr}(S\Theta)-\log\det(\Theta)+\sum_{i\neq j}P_{\omega_{n}}(|\Theta_{ij}|)\\
\text{Tr}(S\Sigma^{-1})-\log\det(\Sigma^{-1})+\sum_{i\neq j}P_{\omega_{n}}(|\Sigma_{ij}|)
\end{align*}
 yields the Graphical LASSO and covariance LASSO, respectively. 
\end{comment}

\begin{comment}
\textbf{Some comments: 1. Problem convex in $\Theta$. 2. How to formulate
the EM version of thresholding? Solving 
\begin{align*}
\arg\min_{\Sigma}\frac{1}{2}\mathbb{E}\left[\|S-\Sigma\|_{F}^{2}\mid Y,\Sigma\right]+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})\\
\end{align*}
 3. General result for sparse covariance in GLM models. 4. Convex+concave
structure, as in Tibshirani. }
\end{comment}

Observe that the first order condition of
\begin{align*}
\min_{\Sigma}\mathbb{E}\left[\text{Tr}(S\Sigma^{-1})-\log\det(\Sigma^{-1})\mid Y,\Sigma^{(m)}\right]
\end{align*}
which is convex in $\Sigma^{-1}$, is exactly the update formula for
the EM algorithm
\begin{align*}
\hat{\Sigma} & =\mathbb{E}\left[S\mid Y,\Sigma^{(m)}\right]\\
 & =\frac{1}{n}\sum_{i=1}^{n}\mathbb{E}\left[(Z_{i}-x_{i})(Z_{i}-x_{i})^{T}\mid X,Y,\Sigma^{(m)}\right]
\end{align*}
 

This suggests that to apply the various sparsity methods, we simply
need to replace the sample covariance with their conditional versions
in the corresponding problems, given observed data and current estimate
of the parameter $\Sigma^{(m)}$, and solve it at every maximization
step of the EM algorithm. 

For example, the EM algorithm applied to probit MLE penalized with
LASSO penality on $\Sigma^{-1}$, 
\begin{align*}
\max_{\beta,\Sigma}\log L(X,Y\mid\beta,\Sigma)-\sum_{i\neq j}P_{\omega_{n}}(|(\Sigma^{-1})_{ij}|)
\end{align*}
becomes 
\begin{align*}
\min_{\Theta}\mathbb{E}\left[\text{Tr}(S\Theta)-\log\det(\Theta)+\sum_{i\neq j}P_{\omega_{n}}(|\Theta_{ij}|)\mid X,Y,\Sigma^{(m)}\right]
\end{align*}
 and since the objective is linear in $S$ this simplifies to 
\begin{align}
\min_{\Theta}\text{Tr}(\mathbb{E}\left[S\mid X,Y,\Sigma^{(m)}\right]\Theta)-\log\det(\Theta)+\sum_{i\neq j}P_{\omega_{n}}(|\Theta_{ij}|)
\end{align}
which is convex in $\Theta$. So we are in effect iteratively solving
graphical LASSO problems with the sample covariance matrix replaced
by the conditional sample covariance given observed variables and
current parameter estimate $\Sigma^{(m)}$.

Similarly, the EM algorithm applied to probit MLE penalize with LASSO
penaltiy on $\Sigma$, 
\begin{align*}
\max_{\beta,\Sigma}\log L(X,Y\mid\beta,\Sigma)-\sum_{i\neq j}P_{\omega_{n}}(|(\Sigma)_{ij}|)
\end{align*}
 becomes 
\begin{align*}
\min_{\Sigma}\text{Tr}(\mathbb{E}\left[S\mid X,Y,\Sigma^{(m)}\right]\Sigma)+\log\det(\Sigma)+\sum_{i\neq j}P_{\omega_{n}}(|\Sigma_{ij}|)
\end{align*}
 which is the covariance LASSO problem with the sample covariance
matrix replaced by the conditional sample covariance given observed
variables and current parameter estimate $\Sigma^{(m)}$. This problem,
however, is non-convex in $\Sigma$, unlike the analogue for $\Theta$.
It is still possible to solve it, e.g. using the MM algorithm proposed
by \cite{bien2011sparse}, but since we need to solve a sequence of
such problems, the LASSO problem with covariance matrix will be much
less efficient to solve compared to the LASSO problem with inverse
covariance matrix. This is part of the reason why we turn to banding
and thresholding methods for sparse covariance matrix estimation. 

The EM algorithm applied to the banding/thresholding penalized regression
problem 
\begin{align*}
\hat{\Sigma} & =\arg\min_{\Sigma}\frac{1}{2}\mathbb{E}\left[\|S-\Sigma\|_{F}^{2}\mid X,Y,\Sigma\right]+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})
\end{align*}
 yields the iteration 
\begin{align*}
\min_{\Sigma}\frac{1}{2}\mathbb{E}\left[\|S-\Sigma\|_{F}^{2}\mid X,Y,\Sigma^{(m)}\right]+\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})
\end{align*}
which is again convex in $\Sigma$, and the solution has the form
\begin{align}
\Sigma^{(m+1)} & =\begin{cases}
S_{ij}^{(m)} & \text{if }i=j\\
h(S_{ij}^{(m)};\omega_{n}) & \text{if }i\neq j
\end{cases}
\end{align}
 where 
\begin{align*}
S^{(m)} & =\mathbb{E}\left[S\mid X,Y,\Sigma^{(m)}\right]
\end{align*}
 is again the conditional sample covariance, and $h$ is the thresholding/banding
operation associated with the penalty $P_{\omega_{n}}(\Sigma_{ij})$.
We recall some popular choices of $h$:
\begin{itemize}
\item Hard thresholding uses $h(z;\omega_{n})=z\cdot1\{|z|\geq\omega_{n}\}$.
\item Soft thresholding uses $h(z;\omega_{n})=\text{sgn}(z)(|z|-\omega_{n})_{+}$. 
\item Banding uses $h(S_{ij};\omega_{n})=0$ if $|i-j|>\omega_{n}$.
\end{itemize}
Thus banding/thresholding methods also directly generalize to the
probit case, and all we need to do is to replace sample covariance
with its conditional version and iterate.

For the horizontal regression problem for probit,
\begin{align*}
\min_{\alpha_{j}\in\mathbb{R}^{m-1}}\frac{1}{2n}\sum_{i}\mathbb{E}\left[|Z_{ij}-Z_{i(-j)}\alpha_{j}|^{2}\mid X,Y,\Sigma\right]+\lambda_{j}\|\alpha_{j}\|_{1}
\end{align*}
it is less clear what form its EM version takes. However, if we instead
solve 
\begin{align*}
\min_{\alpha_{j}\in\mathbb{R}^{m-1}}\frac{1}{2n}\sum_{i}|\mathbb{E}\left[\left(Z_{ij}-Z_{i(-j)}\alpha_{j}\right)\mid X,Y,\Sigma\right]|^{2}+\lambda_{j}\|\alpha_{j}\|_{1}
\end{align*}
the horizontal regression method can be directly generalized: at each
iteration, for each $j$, we compute the conditional means 
\begin{align*}
Z_{ij}^{(m)} & =\mathbb{E}\left[Z_{ij}\mid X,Y,\Sigma^{(m)}\right]
\end{align*}
 for all $i$, and then solve the horizontal regression problem
\begin{align*}
\min_{\alpha_{j}\in\mathbb{R}^{m-1}}\frac{1}{2n}\sum_{i}|Z_{ij}^{(m)}-Z_{i(-j)}^{(m)}\alpha_{j}|^{2}+\lambda_{j}\|\alpha_{j}\|_{1}
\end{align*}
 and update the $j$th column of $\Theta^{(m)}$ using $\alpha_{j}$.

In summary, the update formulae that we derived in this section can
all be obtained as results of applying EM algorithms to optimize appropriate
penalized maximum likelihood or penalized regression problems in the
probit model. 

\textbf{}%
\begin{comment}
\textbf{The sparsity penalty also have a regularizing effect. The
original MLE problem suffers from the identification problem, and
transforming it to an identifiable system rendered the covariance
matrix uninterpretable, and also destroyed any sparsity structure
of $\Sigma$. With the penalized MLE problem, the penalty is effectively
``selecting'' among all the MLE solution pairs $(\theta,\Sigma)$
the one with the most sparse $\Sigma$. Mathematically, because of
the convexity of the penalty terms, the penalized MLE will often be
strictly concave in $(\theta,\Sigma)$, hence has a unique maximizer.
Thus encouraging sparsity not only helps us recover the substantive
relationships among components in a probit model, but also conveniently
circumvents the identification problem in the original MLE problem. }
\end{comment}

In the implemention of the proposed algorithms, we still need to use
Monte Carlo methods to draw samples from the posterior distribution
\begin{align*}
\mathbb{P}(Z_{i}\mid Y_{i},\Sigma^{(m)})
\end{align*}
 For this task, Gibbs sampling is the method of choice, since as discussed
earlier rejection sampling can be slow and the GHK algorithm does
not allow one to draw samples from the posterior distribution easily. 

We also observe that the precision matrix estimation algorithms integrate
nicely with Gibbs sampling, in the following way. Recall that in Gibbs
sampling, we cycle through components of the latent variable and draw
each component conditional on the other entries. In probit models,
this conditional distribution has the following simple form in terms
of the precision matrix $\Theta$:
\begin{align*}
Z_{ij} & \sim\mathcal{N}_{trunc}(\alpha_{j}^{T}Z_{-j},\sigma_{j}^{2},Y_{i})
\end{align*}
where
\begin{align*}
\sigma_{j}^{-2} & =\Theta_{jj}\\
-\sigma_{j}^{-2}\alpha_{j} & =\Theta_{-j,j}
\end{align*}
 and $\mathcal{N}_{trunc}$ denotes truncated normal conditional on
$Y_{i}$. Thus at the $m$th iteration of the EM algorithm, we may
carry out Gibbs sampling using only $\Theta^{(m)}$ and not $\Sigma^{(m)}$
in the Expectation step, and obtain the updated $\Theta^{(m+1)}$
using either Graphical LASSO or horizontal regression. The advantage
of this sampling scheme is that it avoids matrix inversion at each
iteration of the EM algorithm, which both brings computational errors
and increase computation time. 

In our algorithm iterations, we propose to draw only one (or a few)
samples of the latent variable for example rejection sampling or Gibbs
sampling with only a few iterates of the chain. The resulting algorithms
then have the simple form of alternating between drawing latent samples
and using those samples to perform sparse covariance/precision matrix
estimation. 

It has been suggested \cite{natarajan2000monte} that the number of
MCMC samples should increase with the number of iterates. Since the
convergence of MC-EM algorithms depends on approximating the posterior
expectation with high accuracy, using only a few MCMC samples of the
latent variables at every iteration of the EM algorithm is not guaranteed
to lead to its convergence. We note however that in our implementations,
one or a few samples every iteration usually yielded sequences of
estimates that seemed to converge to or at least fluctuate around
the ground truth parameters. 

We speculate that this could be due to two reasons. First, when the
true model is sparse, applying sparsity methods during iterations
of the EM algorithm and thus filtering out noise from signal has the
added benefit that it speeds up convergence by requiring less accuracy
in the approximation of posterior distributions, i.e. requiring fewer
draws of the latent variables. Second, when an EM algorithm reduces
to an update formula that is linear in the posterior moments of the
latent variables, drawing few samples to approximate the moment could
still lead to convergence due to the special structure. This is another
point we plan to investigate further.

In summary, here are the methods that we propose to solve the sparse
covariance/precision matrix in probit models:
\begin{lyxalgorithm}
For sparse covariance matrix estimation, at the $m$th step approximate
$S^{(m)}=\mathbb{E}\left[S\mid X,Y,\Sigma^{(m)}\right]$ with Monte
Carlo methods and then apply thresholding or banding methods to $S^{(m)}$
to obtain $\Sigma^{(m+1)}$.

For sparse precision matrix estimation with graphical LASSO, at the
$m$th step approximate $S^{(m)}=\mathbb{E}\left[S\mid X,Y,\Sigma^{(m)}\right]$
with Monte Carlo methods and then solve the graphical LASSO objective
with $S^{(m)}$ in place of $S$ to obtian $\Theta^{(m+1)}$, which
is inverted to obtain $\Sigma^{(m+1)}$.

For sparse precision matrix estimation with horizontal regression,
at the $m$th step draw a sample of $Z_{i}$ for each $i$, and then
form the $n\times m$ matrix $[Z_{1}\text{ }Z_{2}\text{ }\dots\text{ }Z_{m}]$
and perform horizontal regression to obtain $\Theta^{(m+1)}$, which
is inverted to obtain $\Sigma^{(m+1)}$.

Alternatively, if using Gibbs sampling for sparse precision matrix
estimation, we can directly generate samples $Z_{i}$ conditional
on $Y_{i}$ and $\Theta^{(m)}$, using the formula
\begin{align*}
Z_{ij} & \sim\mathcal{N}_{trunc}(\alpha_{j}^{T}Z_{-j},\sigma_{j}^{2},Y_{i})
\end{align*}
where
\begin{align*}
\sigma_{j}^{-2} & =\Theta_{jj}^{(m)}\\
-\sigma_{j}^{-2}\alpha_{j} & =\Theta_{-j,j}^{(m)}
\end{align*}
\end{lyxalgorithm}
Even though the algorithms we propose here can all be interpreted
as EM algorithms applied to different penalized objectives, they can
also be applied to other estimation methods that do not have a maximum
likelihood/regression formulation. The idea of alternating between
drawing latent variables and performing inference can be applied to
any estimation method that uses the latent variables for inference.
Moreover, in the EM algorithm, there are cases when the full likelihood
is easy to maximize, but the result of the expectation step is not,
so that the maximization step is hard to perform. In this case, the
alternating approach may be much easier to implement than a standard
EM algorithm. Whether there is convergence or if the convergence quantity
is meaningful should be assessed based on the specific model, and
convergence results under general conditions should be investigated
further. 

\begin{comment}
It should be noted that our algorithm performs much better when we
normalize $\Sigma$ to be correlation matrix after every iteration. 
\end{comment}

Since MLE estimator is consistent, with enough observations we should
converge to the population covariance. So one may object that if the
true model is sparse, we should be able to recover such a structure
without imposing the sparsity penalties. There are several problems
with this argument. First, that is assuming a large number of observations.
Second, and more importantly, the identification problem with the
unrestricted covariance matrix may prevent us from obtaining a sparse
MLE estimate: estimating the unidentified system directly can lead
to a non-sparse estimate, whereas estimating the reduced identified
system leads to a non-sparse estimate. Third, convergence of MC-EM
algorithms requires that enough Monte Carlo samples are drawn at each
EM iteration. The reason that the non-penalized EM estimates are non-sparse
could also be because we are only using a few Monte Carlo samples
at each EM iteration. In this regime, thresholding works well and
seems to result in a converging sequence of estimates that are sparse.
The reason of this effectiveness should be addressed. For now, we
simply note that the fact that \emph{regularization} helps with convergence
is a a routinely observed phenomenon in machine learning contexts. 

Finally, to obtain a sparse estimation of the covariance or precision
matrix in the probit model, one may think that it is sufficient to
apply the sparsity methods at the end of the EM algorithm instead
of at every iteration. However, the problem is that due to the accumulation
of simulation and estimation errors, the sparsity of the estimates
are overwhelmed by the accumulated error, so that EM algorithm converges
to a matrix with spurious non-zero entries. This has been observed
in practice for example for estimates of the covariance matrix with
no thresholding. Even with hard thresholding, this problem persists,
and is only alleviated with soft thresholding. 

\subsection{Bayesian Optimization with Simulated Likelihood}

The key to most frequentist approaches to the MLE of the probit model
consists of two parts. The first is an efficient approximation of
the choice probabilities, or equivalently efficient draws of latent
variables conditional on observed variables and model parameters,
using Monte Carlo methods. The second is an optimization problem,
for example direct maximization of simulated likelihood via Newton
or BFGS, minimization of a weighted quadratic form in the method of
simulated moments, and the maximization step in the EM type algorithms.

In this section, we propose to apply a Bayeisan optimization method
\cite{zhou2014gradient} that directly solves the maximum likelihood
problem of the probit model. This method still requires efficient
evaluation of the likelihood given observed variables and parameters,
which can be achieve for example with the GHK algorithm, Gibbs sampling,
or the algorithm proposed in \cite{li2015efficient}. The second step
is a direct maximization of the likelihood via a Bayesian optimization
approach proposed in \cite{zhou2014gradient}.

The Bayesian optimization algorithm is a gradient based stochastic
search algorithm that can be applied to any non-differentiable non-convex
optimization problem
\begin{align*}
\max_{x}H(x)
\end{align*}
 as long as $H(x)$ is bounded below and one can efficiently query
the value of objective function given specific parameter $x$. The
algorithm can be viewed as a form of generalized Robbins-Monro \cite{robbins1951stochastic}
algorithm. In this section we give a self-contained summary of the
main idea of the algorithm.

The key idea is to average the objective by integrating it against
a smooth probability density function parameterized by $\theta$,
giving 
\begin{align*}
\int H(x)f(x;\theta)dx
\end{align*}
 which is smooth in $\theta$. The algorithm alternates between drawing
samples $x_{i}$ from $f(x;\theta)$ and using the samples to update
parameter $\theta$ in a Newton step, with the guarantee that $f(x;\theta)$
becomes more and more concentrated on the set of global optima of
$H$. In practice $f(x;\theta)$ is taken to be a normal distribution,
and so we may see smoothing as a convolution. 

To be more precise, consider $f$ in the family of exponential distributions,
i.e. 
\begin{align*}
f(x) & =\exp(\theta^{T}T(x)-\phi(\theta))
\end{align*}
 and let 
\begin{align*}
L(\theta) & :=\int H(x)f(x;\theta)dx
\end{align*}
 Then we have 
\begin{align*}
\max L(\theta) & \leq\max H(x)=H^{\ast}
\end{align*}
 with equality if and only if the parameterized set of distributions
$f(x;\theta)$ contains an element that is supported on the set of
global optima of $H(x)$.

To maximize the objective $L(\theta)$, a natural idea is to apply
Newton update to $\theta$ via 

\begin{align*}
\theta^{k+1} & =\theta^{k}+(\nabla_{\theta}^{2}L(\theta))^{-1}(\nabla_{\theta}L(\theta))
\end{align*}

This algorithm only requires one to be able to efficiently evaluate
the value of the objective at given parameter values, a task we can
achieve with GHK, Gibbs Sampling, or other sampling methods in the
first step. %
\begin{comment}

\subsection{Issues in Monte Carlo EM}

https://pdfs.semanticscholar.org/d08f/c5afc83b482d30da9928d18e4a445c922335.pdf

\subsection{More efficient sampling of multivariate truncated normal}

\subsection{What does machine learning teach us?}

Method of moments estimator amounts to minimizing a weighted quadratic
distance between observed choice and model choice probabilities. 

Cross entropy loss is another distance measure between two probabilities
that is often used in multinomial logit models. Given simulated choice
probabilities, can we use this objective instead of the method of
moment objective? 
\end{comment}


\section{Empirical Analyses}

\begin{comment}

\subsection{A variant of MC-EM algorithm}

The following lists a couple of empirical results using our proposed
MC-EM algorithm with rejection sampling. Note that we are normalizing
the estimated covariance matrix to correlation matrix at every iteration.
The sample size is 5000 and number of iterations is 1000. 

With standard covariance estimator: 

\begin{align*}
\Sigma & =\begin{bmatrix}1 & 1 & 0\\
1 & 1 & 0\\
0 & 0 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.99 & -0.002\\
0.99 & 1 & -0.007\\
-0.002 & -0.007 & 1
\end{bmatrix}
\end{align*}

\begin{align*}
\Sigma & =\begin{bmatrix}1 & 0.5 & -0.5\\
0.5 & 1 & 0\\
-0.5 & 0 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.49 & -0.71\\
0.49 & 1 & -0.05\\
-0.71 & -0.05 & 1
\end{bmatrix}
\end{align*}
\begin{align*}
\Sigma & =\begin{bmatrix}1 & 0.5 & 0.5\\
0.5 & 1 & 0.5\\
0.5 & 0.5 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.50 & 0.52\\
0.50 & 1 & 0.49\\
0.52 & 0.49 & 1
\end{bmatrix}
\end{align*}

\begin{align*}
\Sigma & =\begin{bmatrix}1 & 0.5 & -0.2\\
0.5 & 1 & 0.5\\
-0.2 & 0.5 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.48 & -0.20\\
0.48 & 1 & 0.49\\
-0.20 & 0.49 & 1
\end{bmatrix}
\end{align*}

With graphical lasso covariance estimator:
\begin{align*}
\Sigma & =\begin{bmatrix}1 & 1 & 0\\
1 & 1 & 0\\
0 & 0 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.99 & 0.01\\
0.99 & 1 & -0.002\\
0.01 & -0.002 & 1
\end{bmatrix}
\end{align*}

\begin{align*}
\Sigma & =\begin{bmatrix}1 & 0.5 & -0.5\\
0.5 & 1 & 0\\
-0.5 & 0 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.47 & -0.41\\
0.47 & 1 & 0.10\\
-0.41 & 0.10 & 1
\end{bmatrix}
\end{align*}

\begin{align*}
\Sigma & =\begin{bmatrix}1 & 0.5 & 0.5\\
0.5 & 1 & 0.5\\
0.5 & 0.5 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.51 & 0.47\\
0.51 & 1 & 0.48\\
0.47 & 0.48 & 1
\end{bmatrix}
\end{align*}

\begin{align*}
\Sigma & =\begin{bmatrix}1 & 0.5 & -0.2\\
0.5 & 1 & 0.5\\
-0.2 & 0.5 & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1 & 0.52 & -0.19\\
0.52 & 1 & 0.49\\
-0.19 & 0.49 & 1
\end{bmatrix}
\end{align*}

\begin{align*}
\Sigma & =\begin{bmatrix}1 &  & 0.65\\
 & 1 &  & 0.58\\
0.65 &  & 1\\
 & 0.58 &  & 1\\
 &  &  &  & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1\\
0.017 & 1\\
\boldsymbol{0.64} & -0.04 & 1\\
0.02 & \boldsymbol{0.58} & 0.01 & 1\\
0.02 & -0.004 & 0.02 & -0.1 & 1
\end{bmatrix}
\end{align*}

The advantage of this iterative algorithm is in exploiting the sparsity
structure of the underlying covariance matrix. If it is sparse, it
is easier to draw from the joint distribution. One natural idea is
then to threshold the entries to retain only those that are above
a certain magnitude. The problem is that this cannot be done at every
iteration, as this prevents the non-zero entries from growing large.
The following shows estimation result of thresholding every 10 iterations.
\begin{align*}
\Sigma & =\begin{bmatrix}1 &  &  & 0.57\\
 & 1\\
 &  & 1\\
 &  &  & 1\\
 & 0.57 &  &  & 1
\end{bmatrix}\\
\hat{\Sigma} & =\begin{bmatrix}1\\
0.006 & 1\\
-0.02 & 0.12 & 1\\
-0.04 & -0.01 & -0.08 & 1\\
0.06 & 0.56 & 0.05 & 0.04 & 1
\end{bmatrix}
\end{align*}
\end{comment}
{} %
\begin{comment}
Still, this ad hoc thresholding is not exclusive to our algorithm.
We can add it to any iterative algorithm like the MC-EM of Natarajan.
So what is the advantage of our approach?

Instrumental variables:

At Cruise, they want to find causal variables that cause a human takeover
of the autonomous car. For each takeover, they have engineers review
and determine the cause of the takeover, usually a subset of a set
of 20 categories. Available to us is about 200 system/environmental
variables. For example, we know how much error the AV's prediction
of the surrounding objects' position and velocity has compared to
ground truth, and if at an intersection, what type of turn it is.
I am charged with determing which of these variables are likely to
be causal. If we want to use an IV approach, seems like we need to
first do a variable selection step followed by 2SLS. Is there any
principled way to find instruments, without domain-specific knowledge?
\end{comment}

We conduct simulation studies for different sizes of choice sets and
compare the speed and accuracy of our proposed algorithms. The details
of the simulation is as follows: we generate $n\times1$ design matrix
from uniform distribution $[-0.5,0.5]$, and generate random error
from multivariate Gaussian centered at 0 with covariate matrix $\Sigma$.
We use $\Sigma$ with different types of structures: 
\begin{enumerate}
\item All off-diagonal entries of $\Sigma$ are non-zero and of the same
value. 
\item Few random off-diagonal entries of $\Sigma$ are non-zero and of the
same value.
\item Few random off-diagonal entries of $\Sigma$ are non-zero and of different
values. 
\end{enumerate}
To facilitate comparisons, we restrict $\Sigma$ to be a correlation
matrix, and impose this restriction on the estimations of the different
algorithms as well. 

\subsection{Thresholding for sparse covariance matrix estimation}

We examine the estimates of some covariance matrices given by the
following methods applied to the MC-EM method with one rejection sampling
during each iteration of the EM algorithm:
\begin{enumerate}
\item Sample covariance matrix.
\item Hard thresholding on sample covariance matrix.
\item Soft thresholding on sample covariance matrix with $h(z;\omega_{n})=\text{sgn}(z)(|z|-\omega_{n})_{+}$. 
\end{enumerate}
We also found that performing thresholding once every $k$ iterations
of the EM algorithm yields better performance than applying it at
every iteration. The intuition is that for true large entries of the
covariance matrix to emerge, the EM algorithm may need to run for
a few iterations. If we perform thresholding at every iteration, even
true signals may be clipped and not given enough chance to emerge.
It is therefore of theoretical and empirical importance to study the
optimal frequency at which to perform thresholding during the EM algorithm. 

\begin{table}
\begin{centering}
\hspace*{-3cm}%
\begin{tabular}{|c|c|c|}
\hline 
ground truth & no LASSO & LASSO\tabularnewline
\hline 
\hline 
$\begin{bmatrix}1 & 0.5\\
 & 1\\
 &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.45 & 0.11\\
 & 1 & 0.07\\
 &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.45 & 0.06\\
 & 1 & -0.003\\
 &  & 1
\end{bmatrix}$\tabularnewline
\hline 
$\begin{bmatrix}1\\
 & 1\\
 &  & 1 & -0.53\\
 &  &  & 1\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & -0.11 & -0.16 & -0.14 & 0.01\\
 & 1 & -0.42 & 0.24 & -0.07\\
 &  & 1 & -0.58 & -0.29\\
 &  &  & 1 & 0.10\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & -0.049 & -0.036 & 0.039 & -0.042\\
 & 1 & 0.043 & 0.039 & -0.070\\
 &  & 1 & -0.56 & -0.016\\
 &  &  & 1 & -0.03\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
$\begin{bmatrix}1 & 0.06 &  & 0.37\\
 & 1 &  & 0.16\\
 &  & 1 &  & 0.56\\
 &  &  & 1\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.006 & 0.15 & 0.27 & 0.19\\
 & 1 & 0.25 & 0.24 & 0.13\\
 &  & 1 & 0.19 & 0.46\\
 &  &  & 1 & 0.17\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.13 & -0.02 & 0.32 & -0.04\\
 & 1 & -0.09 & 0.11 & -0.008\\
 &  & 1 & 0.02 & 0.54\\
 &  &  & 1 & 0.05\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
\end{tabular}\hspace*{-2cm}
\par\end{centering}
\caption{Estimates of the inverse covariance matrix in probit models with MLE
and penalized MLE. We used a sample size of 2000. Penalized MLE with
LASSO is estimated at every iteration with $\lambda_{n}=0.1\sqrt{\frac{\log m}{n}}$.
Result is averaged over last 100 iterations of the EM algorithm. We
see that LASSO is able to relatively accurately locate the non-zero
entries and at the same time give good estimates of their values.}
\end{table}

\begin{table}
\noindent \begin{centering}
\hspace*{-3cm}%
\begin{tabular}{|c|c|c|}
\hline 
ground truth & no thresholding & soft thresholding\tabularnewline
\hline 
\hline 
$\begin{bmatrix}1 & 0.5\\
 & 1\\
 &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.52 & -0.06\\
 & 1 & 0.11\\
 &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.46 & -0.04\\
 & 1 & -0.01\\
 &  & 1
\end{bmatrix}$\tabularnewline
\hline 
$\begin{bmatrix}1\\
 & 1\\
 &  & 1 & -0.53\\
 &  &  & 1\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & -0.01 & 0.02 & 0.01 & 0.17\\
 & 1 & -0.13 & 0.01 & 0.20\\
 &  & 1 & -0.45 & -0.09\\
 &  &  & 1 & -0.03\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & -0.001 & 0.05 & 0.06 & -0.009\\
 & 1 & -0.02 & -0.01 & 0.12\\
 &  & 1 & -0.46 & -0.009\\
 &  &  & 1 & -0.03\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
$\begin{bmatrix}1 &  &  & -0.36\\
 & 1 &  & -0.15\\
 &  & 1 &  & -0.55\\
 &  &  & 1\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.20 & 0.16 & -0.38 & -0.13\\
 & 1 & 0.07 & -0.25 & -0.15\\
 &  & 1 & -0.04 & -0.51\\
 &  &  & 1 & 0.21\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.004 & 0.06 & -0.40 & 0.01\\
 & 1 & 0.09 & -0.02 & -0.03\\
 &  & \boldsymbol{} & -0.14 & -0.42\\
 &  &  & 1 & 0.01\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
\end{tabular}\hspace*{-2cm}
\par\end{centering}
\caption{Estimates of the covariance matrix in probit models with MLE and penalized
MLE. We used a sample size of 2000. Thresholding is performed once
every 25 iterations of the EM algorithm with $\omega_{n}=3\sqrt{\frac{\log m}{n}}$.
Result is averaged over last 100 iterations of the EM algorithm. We
see that soft thresholding is able to relatively accurately locate
the non-zero entries and at the same time give good estimates of their
values. }
\end{table}

\begin{table}
\begin{centering}
\hspace*{-3cm}%
\begin{tabular}{|c|c|c|}
\hline 
ground truth & no banding & banding\tabularnewline
\hline 
\hline 
$\begin{bmatrix}1 & 0.5\\
 & 1 & 0.5\\
 &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.45 & 0.11\\
 & 1 & 0.07\\
 &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.51 & 0.03\\
 & 1 & 0.55\\
 &  & 1
\end{bmatrix}$\tabularnewline
\hline 
$\begin{bmatrix}1 & 0.2\\
 & 1 & 0.3\\
 &  & 1 & 0.3\\
 &  &  & 1 & 0.2\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & -0.11 & -0.16 & -0.14 & 0.01\\
 & 1 & -0.42 & 0.24 & -0.07\\
 &  & 1 & -0.58 & -0.29\\
 &  &  & 1 & 0.10\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & -0.049 & -0.036 & 0.039 & -0.042\\
 & 1 & 0.043 & 0.039 & -0.070\\
 &  & 1 & -0.56 & -0.016\\
 &  &  & 1 & -0.03\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
$\begin{bmatrix}1 & 0 & 0.08 & 0 & -0.004\\
 & 1 & 0 & -0.02 & 0.02\\
 &  & 1 & -0.005 & -0.45\\
 &  &  & 1 & 0\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.006 & 0.15 & 0.27 & 0.19\\
 & 1 & 0.25 & 0.24 & 0.13\\
 &  & 1 & 0.19 & 0.46\\
 &  &  & 1 & 0.17\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.13 & -0.02 & 0.32 & -0.04\\
 & 1 & -0.09 & 0.11 & -0.008\\
 &  & 1 & 0.02 & 0.54\\
 &  &  & 1 & 0.05\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
\end{tabular}\hspace*{-2cm}
\par\end{centering}
\caption{Estimates of the covariance matrix in probit models with MLE and banding.
We used a sample size of 2000. Banding is performed once every 25
iterations of the EM algorithm with $\omega_{n}=1$. Result is averaged
over last 100 iterations of the EM algorithm. We see that banding
is able to relatively accurately locate the non-zero entries and at
the same time give good estimates of their values. }
\end{table}

\begin{table}
\begin{centering}
\hspace*{-3cm}%
\begin{tabular}{|c|c|c|}
\hline 
Thresholding & LASSO & Banding\tabularnewline
\hline 
\hline 
$\begin{bmatrix}1 & 0 & 0.08 & 0 & -0.004\\
 & 1 & 0 & -0.02 & 0.02\\
 &  & 1 & -0.005 & -0.45\\
 &  &  & 1 & 0\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.17 & 0 & 0.31 & -0.01\\
 & 1 & -0.04 & 0.13 & 0\\
 &  & 1 & 0.06 & 0.51\\
 &  &  & 1 & 0.08\\
 &  &  &  & 1
\end{bmatrix}$ & $\begin{bmatrix}1 & 0.12 & 0 & 0 & 0\\
 & 1 & 0.16 & 0 & 0\\
 &  & 1 & 0.37 & 0\\
 &  &  & 1 & 0.16\\
 &  &  &  & 1
\end{bmatrix}$\tabularnewline
\hline 
\end{tabular}\hspace*{-2cm}
\par\end{centering}
\caption{Some intermediate estimates demonstrating the effect of sparsity penalties. }
\end{table}


\section{Consistency of Sparse Covariance Estimators}

In this section, we discuss the statistical properties of the covariance/precision
matrix estimators based on the sparsity penalized maximum likelihood
approach. We show the estimation consistency of penalty based estimators
with convergence rates, as well as their model selection consistency.
The proof is based on ideas from \cite{rothman2008sparse} and \cite{lam2009sparsistency}.

Convergence in log-likelihood: With appropriate penalty strength,
all local minimizers will have log likelihood converging to the log
likelihood of the true parameter. 

\subsection{Estimation Consistency }

\textbf{}%
\begin{comment}
\textbf{First show the consistency of MLE for regular probit models. }
\end{comment}

\begin{comment}
Discuss the asymptotics of the corresponding penalized MLE estimator--
in the large sample limit, converges to the matrix obtained from the
corresponding methods applied to the population covariance? In the
special case, does the MLE converge to the population?

c.f. Knight and Fu 2000

The hope for consistency of any penalized maximum likelihood estimators
relies on the true parameters exhibiting the corresponding structures
encouraged by the penalty term. 
\end{comment}

\begin{thm}
(estimation consistency of precision LASSO for probit) Suppose $X_{i}\perp\epsilon_{i}$
has continuous pdf with compact support $[-M,M]^{p}$. With the penalty
strength
\begin{align*}
\lambda_{n} & =C\sqrt{\frac{\log m}{n}}
\end{align*}
and sparsity parameter 
\begin{align*}
s & :=|\mathcal{S}|\\
\mathcal{S} & :=\{(i,j):\Theta_{ij}^{0}\neq0,i\neq j\}
\end{align*}
 where the positive definite $\Theta^{0}$ is the true covariance
matrix, there exists a local maximizer $(\hat{\beta},\hat{\Theta}_{\lambda_{n}})$
of the penalized likelihood
\begin{align*}
\max_{\beta,\Sigma}\frac{2}{n}\log L(X,Y\mid\beta,\Theta)-\lambda_{n}\sum_{i\neq j}|\Theta_{ij}|
\end{align*}
 such that 
\begin{align*}
\|\hat{\Theta}_{\lambda_{n}}-\Theta^{0}\|_{F} & =O_{P}(\sqrt{\frac{(m+s)\log m}{n}})
\end{align*}
\end{thm}
\begin{proof}
Denote the negative penalized likelihood by 
\begin{align*}
Q(\Theta) & =-\frac{2}{n}\log L(X,Y\mid\beta,\Theta)+\lambda_{n}\sum_{i\neq j}|\Theta_{ij}|
\end{align*}
omitting the dependence on data and $\beta$. 

Consider the set $\mathcal{A}=\{\Delta:\Delta=\Delta^{T},\|\Delta\|_{F}=C\sqrt{\frac{(m+s)\log m}{n}}\}$.
The key of the proof is to show that 
\begin{align*}
\mathbb{P}(\inf_{\Delta\in\mathcal{A}}Q(\Theta^{0}+\Delta))>Q(\Theta^{0})) & \rightarrow1
\end{align*}
 Since $\Theta^{0}\in\{\Theta^{0}+\Delta:\Delta=\Delta^{T},\|\Delta\|_{F}<C\sqrt{\frac{(m+s)\log m}{n}}\}$,
this implies that there exists a local minimum $\hat{\Theta}_{\lambda_{n}}$
of $Q$ that satisfies 
\begin{align*}
\|\hat{\Theta}_{\lambda_{n}}-\Theta^{0}\|_{F} & =O_{P}(C\sqrt{\frac{(m+s)\log m}{n}})
\end{align*}

For any $\Theta=\Theta^{0}+\Delta$ where $\Delta\in\mathcal{A}$,
write the difference in likelihood
\begin{align*}
Q(\Theta)-Q(\Theta^{0}) & =I_{1}+I_{2}+I_{3}
\end{align*}
 where 
\begin{align*}
I_{1} & =-\frac{2}{n}\sum_{i}\log\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta))dZ_{i}-\log\det(\Theta)\\
 & -(-\frac{2}{n}\sum_{i}\log\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta^{0}))dZ_{i}-\log\det(\Theta_{0}))\\
I_{2} & =\sum_{(i,j)\in S^{c}}(\lambda_{n}|\Theta_{ij}|-\lambda_{n}|\Theta_{ij}^{0}|)\\
I_{3} & =\sum_{(i,j)\in S}(\lambda_{n}|\Theta_{ij}|-\lambda_{n}|\Theta_{ij}^{0}|)
\end{align*}
where $\mathcal{S}=\{(i,j):\Theta_{ij}^{0}\neq0,i\neq j\}$ and $S_{i}=(Z_{i}-X_{i}\beta)(Z_{i}-X_{i}\beta)^{T}$.

Our task is to show that the difference is positive asymptotically
with probability going to 1. 

First, 
\begin{align*}
\log\det(\Theta^{0})-\log\det(\Theta) & =-Tr(\Sigma_{0}\Delta)+\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}
\end{align*}
 where $\otimes$ is the Kronecker product and $\tilde{\Delta}$ is
$\Delta$ vectorized. 

We then have
\begin{align*}
I_{1} & \geq-\frac{2}{n}\sum_{i}\frac{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))\cdot Tr(-\frac{1}{2}S_{i}(\Theta-\Theta_{0}))dZ_{i}}{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))dZ_{i}}\\
 & -Tr(\Sigma_{0}\Delta)+\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}
\end{align*}
\begin{comment}
\begin{proof}
\begin{align*}
I_{1} & =-\frac{2}{n}\sum_{i}\frac{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))\cdot Tr(-\frac{1}{2}S_{i}(\Theta-\Theta_{0}))dZ_{i}}{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))dZ_{i}}\\
 & +\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)\text{derivative of }dv\right]\tilde{\Delta}\\
 & -Tr(\Sigma_{0}\Delta)+\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Omega_{0}+v\Delta)^{-1}\otimes(\Omega_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}
\end{align*}
\end{proof}
\end{comment}
{} by convexity. 

Note that the first term is equal to 
\begin{align*}
\frac{1}{n}\sum_{i}\frac{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))\cdot Tr(S_{i}\Delta)dZ_{i}}{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))dZ_{i}}
\end{align*}
 and each term in the sum 
\begin{align*}
\frac{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta))\cdot Tr(S_{i}\Delta)dZ_{i}}{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta))dZ_{i}}
\end{align*}
 can then be written 
\begin{align*}
Tr(\mathbb{E}_{i}S_{i}\Delta)
\end{align*}
 where $\mathbb{P}_{i}$ is the distribution with density $\frac{\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))}{\int_{A_{i}}\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))dZ_{i}}$
defined on $A_{i}$. 

We can then write 
\begin{align*}
I_{1} & \geq\frac{1}{n}\sum_{i}Tr(\Delta(\mathbb{E}_{i}S_{i}-\Sigma_{0}))\\
 & +\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}\\
 & =Tr(\Delta(S-\Sigma_{0}))+\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}
\end{align*}
 where 
\begin{align*}
S= & \frac{1}{n}\sum_{i}\mathbb{E}_{i}S_{i}
\end{align*}
 is an analogue of the ``sample covariance'' in the probit model.
Since we do not observe the latent variables $Z_{i}$, we take the
expectation with respect to the distribution that is proportional
to $\exp(-\frac{1}{2}Tr(S_{i}\Theta_{0}))$ and supported on $A_{i}$.

\begin{comment}
\begin{proof}
Because $Z_{i}$s are independent truncated normal distributions,
we may write 
\begin{align*}
S & =\mathbb{E}\frac{1}{n}\sum_{i}S_{i}
\end{align*}
 where $\mathbb{E}=\mathbb{E}_{n}\mathbb{E}_{n-1}\cdots\mathbb{E}_{1}$. 

Now recall the lemma above which states that for $Z_{i}$ i.i.d. $\mathcal{N}(0,\Sigma)$,
\begin{align*}
\mathbb{P}(|\frac{1}{n}\sum_{i}Z_{ij}Z_{ik}-\Sigma_{jk}|\geq\nu) & \leq c_{1}\exp(-c_{2}n\nu^{2})\text{ for }|\nu|\leq\delta
\end{align*}
 where $c_{1},c_{2},\delta$ depend on the largest eigenvalue of $\Sigma$. 

Our task is to use this concentration result to show that given $X_{i}$,
the probability distribution $\mathbb{P}$ on $\prod_{i}Y_{i}$ induced
by $X_{i}$ and $\epsilon_{i}\sim\mathcal{N}(0,\Sigma)$ satisfies
\begin{align*}
\mathbb{P}(\prod_{i}Y_{i}:|\frac{1}{n}\sum_{i}\mathbb{E}_{i}((Z_{ij}-X_{ij}\beta)(Z_{ik}-X_{ik}\beta)\mid Y_{i})-\Sigma_{jk}|\geq\nu)
\end{align*}
 decays exponentially in $\nu$. 

First observe that each tuple $(X_{i},Y_{i})$ induces a partition
$\{P_{i}^{j}\}_{j=1}^{m}$ into $m$ subsets of $\mathbb{R}^{m}$,
where elements $Z_{i}$ in the same subset are mapped to the same
value of $Y_{i}$ by the map $\arg\max_{j}Z_{ij}$. The probability
on the left hand side is the product measure of 
\begin{align*}
\otimes\mathcal{N}(X_{i}\beta,\Sigma)
\end{align*}
 on sets of the form 
\begin{align*}
(P_{1}^{j_{1}},P_{2}^{j_{2}},\dots,P_{n}^{j_{n}})
\end{align*}
 where 
\begin{align*}
|\frac{1}{n}\sum_{i}\mathbb{E}_{i}\left[(Z_{ij}-X_{ij}\beta)(Z_{ik}-X_{ik}\beta)\mid P_{i}^{j_{i}}\right]-\Sigma_{jk}| & \geq\nu
\end{align*}

The key observation is that if the measures of $P_{i}^{j}$ are uniformly
bounded below by some constant $\gamma\in(0,1)$ under the measure
$\mathcal{N}(X_{i}\beta,\Sigma)$ for all $i,j$, then at points $\{Z_{i}\}_{i=1}^{n}$
where $|\frac{1}{n}\sum_{i}(Z_{ij}-X_{ij}\beta)(Z_{ik}-X_{ik}\beta)-\Sigma_{jk}|\leq\nu$,
we must have 
\begin{align*}
|\frac{1}{n}\sum_{i}\gamma\left[(Z_{ij}-X_{ij}\beta)(Z_{ik}-X_{ik}\beta)\mid P_{i}^{j_{i}}\right]-\Sigma_{jk}| & \leq\nu
\end{align*}
\end{proof}
\end{comment}

Note that the conditional second moment 
\begin{align*}
\Psi_{i} & =\mathbb{E}\left[S_{i}\mid X_{i},Y_{i}\right]
\end{align*}
 takes on one of $m$ possible values $\{\psi_{i}^{j}\}_{j=1}^{m}$,
with
\begin{align*}
\mathbb{P}(\Psi_{i}=\psi_{i}^{j}) & =\mathbb{P}(A(X_{i},Y_{i}=j))
\end{align*}
 where the map $A:\mathbb{R}^{m\times p}\times\{0,1\}^{m}\rightarrow\mathbb{R}^{m}$
determines the region of $Z_{i}$ that is consistent with $X_{i},Y_{i}$,
and $\mathbb{P}$ is the distribution $\mathcal{N}(X_{i}\beta,\Sigma_{0})$. 

It follows that the expectation of $\Psi_{i}$ is equal to 
\begin{align*}
\sum_{j=1}^{m}\Psi_{i}\cdot\mathbb{P}(A(X_{i},Y_{i}=j)) & =\mathbb{E}(S_{i}\mid X_{i})=\Sigma_{0}
\end{align*}

Our next step is to show that each entry of $\Psi_{i}$ is a bounded
random variable, and then from independence and the expectation calculation
above, Hoeffding's inequality implies 
\begin{align*}
\mathbb{P}(|\frac{1}{n}\sum_{i}\mathbb{E}\left[(Z_{ij}-X_{i}\beta)(Z_{ik}-X_{i}\beta)\mid X_{i},Y_{i}\right]-\Sigma_{0}|\geq\nu) & \leq\exp(-Cn\nu^{2})
\end{align*}
For each $j$, we have 
\begin{align*}
|\mathbb{E}\left[(Z_{ij}-X_{i}\beta)(Z_{ik}-X_{i}\beta)\mid X_{i},Y_{i}=j\right]| & \leq\frac{1}{\mathbb{P}(A(X_{i},Y_{i}=j))}\cdot\sqrt{\Sigma_{jj}^{0}\Sigma_{kk}^{0}}
\end{align*}
To bound $\mathbb{P}(A(X_{i},Y_{i}=j))$, note that by assumption
$X_{i}$ has compact support, so that there exists $\alpha>0$ such
that
\begin{align*}
\mathbb{P}(A(X_{i},Y_{i})) & \geq\alpha
\end{align*}
 and so 
\begin{align*}
\mathbb{P}(|\frac{1}{n}\sum_{i}\mathbb{E}\left[(Z_{ij}-X_{i}\beta)(Z_{ik}-X_{i}\beta)\mid X_{i},Y_{i}\right]-\Sigma_{jk}^{0}|\geq\nu) & \leq2\exp(-\frac{\alpha}{2\max_{i}\Sigma_{ii}^{0}}n\nu^{2})
\end{align*}

Now by symmetry, 
\begin{align*}
|Tr(\Delta(S-\Sigma^{0}))| & \leq|\sum_{i\neq j}(S_{ij}-\Sigma_{ij}^{0})\Delta_{ij}|+|\sum_{i}(S_{ii}-\Sigma_{ii}^{0})\Delta_{ii}|=K_{1}+K_{2}
\end{align*}
 Taking $\nu=C_{1}\sqrt{\frac{\log m}{n}}$ union bound combined with
the concentration result above imply that with probability going to
1, 
\begin{align*}
\max_{i\neq j}|S_{ij}-\Sigma_{ij}^{0}| & \leq C_{1}\sqrt{\frac{\log m}{n}}
\end{align*}
 so that 
\begin{align*}
K_{1} & \leq C_{1}\sqrt{\frac{\log m}{n}}\sum_{i\neq j}|\Delta_{ij}|
\end{align*}
 Similarly, Cauchy-Schwarz combined with the concentration bound imply
that 
\begin{align*}
K_{2} & \leq C_{2}\sqrt{\frac{(m+s)\log m}{n}}\cdot\sqrt{\sum_{i}|\Delta_{ii}|^{2}}
\end{align*}
 with probability going to 1. 

Let $\varphi_{min}(M)=\min_{\|x\|=1}x^{T}Mx$. The second term 
\begin{align*}
\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}
\end{align*}
 in $I_{1}$ satisfies 
\begin{align*}
\tilde{\Delta}^{T}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\tilde{\Delta}\\
\geq\varphi_{\min}\left[\int_{0}^{1}(1-v)(\Theta_{0}+v\Delta)^{-1}\otimes(\Theta_{0}+v\Delta)^{-1}dv\right]\cdot\|\Delta\|_{F}^{2}\\
=\int_{0}^{1}(1-v)\varphi_{\min}^{2}\left((\Theta_{0}+v\Delta)^{-1}\right)dv\cdot\|\Delta\|_{F}^{2}\\
\geq\frac{1}{2}\min_{0\leq v\leq1}\varphi_{\min}^{2}\left((\Theta_{0}+v\Delta)^{-1}\right)\cdot\|\Delta\|_{F}^{2}\\
\geq\frac{1}{2}\min_{\|\Delta\|_{F}\leq C\sqrt{\frac{(m+s)\log m}{n}}}\varphi_{\min}^{2}\left((\Theta_{0}+\Delta)^{-1}\right)
\end{align*}
 Now
\begin{align*}
\varphi_{\min}^{2}\left((\Theta_{0}+\Delta)^{-1}\right) & =\varphi_{\max}^{-2}(\Theta_{0}+\Delta)\\
 & \geq(\|\Theta_{0}\|+\|\Delta\|)^{-2}
\end{align*}
 and since $\|\Delta\|\leq\|\Delta\|_{F}\rightarrow0$, the right
hand side is lower bounded by $\frac{1}{\|\Theta_{0}\|^{2}}=\|\Sigma_{0}\|^{2}$
with probability tending to 1. 

Now for $I_{2}=\sum_{(i,j)\in S^{c}}(\lambda_{n}|\Theta_{ij}|-\lambda_{n}|\Theta_{ij}^{0}|)$
and $I_{3}=\sum_{(i,j)\in S}(\lambda_{n}|\Theta_{ij}|-\lambda_{n}|\Theta_{ij}^{0}|)$,
we have 
\begin{align*}
I_{2} & =\lambda_{n}\sum_{(i,j)\in S^{c}}|\Theta_{ij}|=\lambda_{n}\sum_{(i,j)\in S^{c}}|\Delta_{ij}|\\
I_{3} & \geq-\lambda_{n}\sum_{(i,j)\in S}|\Theta_{ij}-\Theta_{ij}^{0}|=-\lambda_{n}\sum_{(i,j)\in S}|\Delta_{ij}|
\end{align*}

Now if we let 
\begin{align*}
\lambda_{n} & =\frac{C_{1}}{\epsilon}\sqrt{\frac{\log m}{n}}
\end{align*}
 we have 
\begin{align*}
Q(\Theta)-Q(\Theta^{0}) & \geq\|\Sigma_{0}\|^{2}\|\Delta\|_{F}^{2}-C_{1}\sqrt{\frac{\log m}{n}}\sum_{i\neq j}|\Delta_{ij}|-C_{2}\sqrt{\frac{(m+s)\log m}{n}}\cdot\sqrt{\sum_{i}|\Delta_{ii}|^{2}}\\
 & +\lambda_{n}\sum_{(i,j)\in S^{c}}|\Delta_{ij}|-\lambda_{n}\sum_{(i,j)\in S}|\Delta_{ij}|\\
 & \geq\|\Sigma_{0}\|^{2}\|\Delta\|_{F}^{2}-C_{1}\sqrt{\frac{\log m}{n}}(1+\frac{1}{\epsilon})\sum_{(i,j)\in S}|\Delta_{ij}|-C_{2}\sqrt{\frac{(m+s)\log m}{n}}\cdot\sqrt{\sum_{i}|\Delta_{ii}|^{2}}\\
 & \geq\|\Sigma_{0}\|^{2}\|\Delta\|_{F}^{2}-C_{1}\sqrt{\frac{\log m}{n}}(1+\frac{1}{\epsilon})\sqrt{m+s}\cdot\sqrt{\sum_{(i,j)\in S}|\Delta_{ij}|^{2}}-C_{2}\sqrt{\frac{(m+s)\log m}{n}}\cdot\sqrt{\sum_{i}|\Delta_{ii}|^{2}}\\
 & \geq\sum_{(i,j)\in S}|\Delta_{ij}|^{2}\cdot\left(\|\Sigma_{0}\|^{2}-C_{1}\sqrt{\frac{\log m}{n}}(1+\frac{1}{\epsilon})\sqrt{m+s}/\sqrt{\sum_{(i,j)\in S}|\Delta_{ij}|^{2}}\right)\\
 & +\sum_{i}|\Delta_{ii}|^{2}\cdot\left(\|\Sigma_{0}\|^{2}-C_{1}\sqrt{\frac{\log m}{n}}(1+\frac{1}{\epsilon})\sqrt{m+s}/\sqrt{\sum_{i}|\Delta_{ii}|^{2}}\right)>0
\end{align*}
 for $n$ sufficiently large, where we have used $\sum_{(i,j)\in S}|\Delta_{ij}|\leq\sqrt{s}\sqrt{\sum_{(i,j)\in S}|\Delta_{ij}|^{2}}$.
\end{proof}
\begin{comment}
%
\begin{thm}
(estimation consistency of covariance LASSO)
\end{thm}
\textbf{In the future, relax boundedness of $X_{i}$, and show that
e.g. $X_{i}$ independent of $\epsilon_{i}$ and Gaussian leads to
a sub-Gaussian $\Psi_{i}$.}
\begin{thm}
(estimation consistency of thresholding) Suppose we have the system
\begin{align*}
Z_{i1} & =x_{i1}+\epsilon_{i2}\\
Z_{i2} & =x_{i2}+\epsilon_{i2}\\
 & \vdots\\
Z_{im} & =x_{im}+\epsilon_{im}
\end{align*}
where $\epsilon_{i}\sim\mathcal{N}(0,\Sigma)$ i.i.d and we observe
data points 
\begin{align*}
\{(Y_{i},x_{i1},\dots,x_{im})\}_{i=1}^{n}
\end{align*}
and
\begin{align*}
Y_{ij} & =\begin{cases}
1 & \text{if }Z_{ij}=\max_{j}Z_{ij}\\
0 & \text{otherwise}
\end{cases}
\end{align*}
for all $j$. 

Let $\hat{\Sigma}$ be the solution to the hard-thresholding penalized
maximum likelihood maximization 
\begin{align*}
\max_{\Sigma}\log L(X,Y\mid\theta,\Sigma)-\sum_{i\neq j}P_{\omega_{n}}(\Sigma_{ij})\\
\Longleftrightarrow\\
\max_{\Sigma}\sum_{i}\log\int_{A_{i}}f(Z_{i}\mid X_{i},\Sigma)dZ_{i1}\dots dZ_{im}-\sum_{i\neq j}\left(\omega_{n}^{2}-(|\Sigma_{ij}|-\omega_{n})^{2}1\{|\Sigma_{ij}|<\omega_{n}\}\right)
\end{align*}
 with 
\begin{align*}
\omega_{n} & =M'\sqrt{\frac{\log m}{n}}
\end{align*}
 for some sufficiently large $M'$, and $\frac{\log m}{n}=o(1)$.
Then uniformly on the set of sparse matrices 
\begin{align*}
\{\Sigma:\Sigma_{ii}\leq M,\sum_{j=1}^{m}1(\Sigma_{ij}\neq0)\leq c_{0}(m),\forall i\}
\end{align*}
 we have 
\begin{align*}
\|\hat{\Sigma}-\Sigma\| & =O_{P}(c_{0}(m)\sqrt{\frac{\log m}{n}})
\end{align*}
 and 
\begin{align*}
\frac{1}{m}\|\hat{\Sigma}-\Sigma\|_{F}^{2} & =O_{P}(c_{0}(m)\sqrt{\frac{\log m}{n}})
\end{align*}
\end{thm}
\end{comment}


\subsection{Model Selection Consistency}

A different notion of consistency is often studied in model selection
settings, starting with the LASSO. Here we are concerned with whether
an estimator is able to recover the sparsity patterns of the true
covariance matrix with increasing probability. More precisely, model
selection consistency requires 
\begin{align*}
\mathbb{P}(\{(i,j):\hat{\Sigma}_{ij}^{n}\neq0\}=\{(i,j):\Sigma_{ij}\neq0\}\rightarrow1 & \text{ as }n\rightarrow\infty
\end{align*}

\textbf{}%
\begin{comment}
\textbf{c.f. Meinshausen and Buhlmann 2006}
\end{comment}

\begin{thm}
(model selection consistency of precision LASSO) When $s=O(m)$, i.e.
the number of non-zero entries of the true covariance matrix is on
the same order as the number of features, any local maximizer of the
penalized likelihood that satisfies $\|\hat{\Omega}_{\lambda_{n}}-\Omega^{0}\|_{F}=O_{P}(\sqrt{\frac{(m+s)\log m}{n}})$
is model consistent, i.e. with probability tending to 1, $(\Omega_{\lambda_{n}})_{ij}=0$
for all $(i,j)$ such that $\Omega_{ij}^{0}=0$. 
\end{thm}
%
\begin{proof}
Let $\Omega_{\lambda_{n}}$ be any local minimizer of the negative
penalized log-likelihood 
\begin{align*}
Q(\Omega) & =\frac{2}{n}\log L(X,Y\mid\theta,\Omega)+\lambda_{n}\sum_{i\neq j}|\Omega_{ij}|\\
 & =-\log\det(\Omega)-\frac{2}{n}\sum_{i}\log\int_{A_{i}}\exp(-\frac{1}{2}(Z_{i}-X_{i}\beta)^{T}\Omega(Z_{i}-X_{i}\beta))dZ_{i}+\lambda_{n}\sum_{i\neq j}|\Omega_{ij}|
\end{align*}
 that satisfies $\|\hat{\Omega}_{\lambda_{n}}-\Omega^{0}\|_{F}=O_{P}(\sqrt{\frac{(m+s)\log m}{n}})$.
Taking the derivative of the above with respect to $\Omega_{ij}$
with $\Omega_{ij}^{0}=0$, we have 
\begin{align*}
\partial_{\Omega_{ij}}Q(\Omega) & =2(S_{ij}-\Sigma_{ij}+\lambda_{n}\text{sgn}(\Omega_{ij}))
\end{align*}
where again 
\begin{align*}
S & =\frac{1}{n}\sum_{i}\mathbb{E}_{i}S_{i}
\end{align*}
 and $\mathbb{P}$ is the truncated normal supported on $A_{i}$.
The idea of the proof is to show that with probability going to 1,
the sign of $\partial_{\Omega_{ij}}Q(\Omega)$ is equal to $\text{sgn}(\Omega_{ij})$,
with convergence independent of $i,j$. Since $\partial_{\Omega_{ij}}Q(\Omega)=0$
at local optima, $\text{sgn}(\Omega_{ij})$ will be equal to 0 for
all $i,j$ with probability going to 1. Thus we need to estimate the
order of $S_{ij}-\Sigma_{ij}$ independent of $i,j$. We have 
\begin{align*}
S_{ij}-\Sigma_{ij} & =I_{1}+I_{2}\\
I_{1} & =S_{ij}-\Sigma_{ij}^{0}\\
I_{2} & =\Sigma_{ij}^{0}-\Sigma_{ij}
\end{align*}

By standard concentration results, we have 
\begin{align*}
\max_{i,j}|S_{ij}-\Sigma_{ij}^{0}| & =O_{P}(\sqrt{\frac{\log m}{n}})
\end{align*}
 On the other hand, since 
\begin{align*}
|\Sigma_{ij}-\Sigma_{ij}^{0}| & \leq\|\Sigma-\Sigma_{0}\|\\
 & \leq\|\Sigma-\Sigma_{0}\|_{F}\\
 & =\|\Sigma(\Omega-\Omega_{0})\Sigma_{0}\|_{F}\\
 & \leq\|\Sigma\|\cdot\|\Omega-\Omega_{0}\|\cdot\|\Sigma_{0}\|=O(\|\Omega-\Omega_{0}\|)
\end{align*}
 since 
\begin{align*}
\|\Sigma\| & =\lambda_{\min}^{-1}(\Omega)\leq(\lambda_{\min}(\Omega_{0})+\lambda_{\min}(\Omega-\Omega_{0}))^{-1}
\end{align*}
 and 
\begin{align*}
\lambda_{\min}(\Omega-\Omega_{0}) & \leq\|\Omega-\Omega_{0}\|_{F}\\
 & =O_{P}(\sqrt{\frac{(m+s)\log m}{n}})\\
 & =O_{P}(\sqrt{\frac{m\log m}{n}})\\
 & =o_{P}(1)
\end{align*}
Therefore we have 
\begin{align*}
\max_{ij}|\Sigma_{ij}-\Sigma_{ij}^{0}| & =O_{P}(\sqrt{\frac{\log m}{n}}+\sqrt{\frac{m\log m}{n}})\\
 & =O_{P}(\sqrt{\frac{m\log m}{n}})
\end{align*}
 On the other hand, we have 
\begin{align*}
\lambda_{n} & =O_{P}(\sqrt{\frac{(m+s)\log m}{n}})=O_{P}(\sqrt{\frac{m\log m}{n}})
\end{align*}
 and the result follows.
\end{proof}


\section{Conclusion }
In this paper, we developed penalized maximum likelihood and penalized
regression methods for estimating sparse covariance matrices in probit
models. These model selection approaches allow us to flexibly impose
prior information on the structure of the covariance matrix, while
at the same time circumventing identification issues with the unnormalized
probit model. We showed the estimation and model selection consistency
of the estimators, and proposed several algorithms for estimating
sparse covariance/precision matrix in probit models based on the Monte
Carlo EM algorithm. These algorithms can also be understood as implementing
the general idea of alternating between drawing latent variables and
solving the optimization problem associated with the non-latent variable
setting. Even though we only sample a few Monte Carlo samples at each
iteration, convergence is generally observed. Numerical experiments
also show that they perform well at locating the non-zero entries
of the covariance/precision matrix, and that they outperform conventional
EM algorithms in terms of accuracy, with no extra overhead on computation
time. 

Penalized likelihood and regression methods are not new. But applied
to the probit model, they have the added benefit of performing model
selection on the unidentified models. They are also not limited to
probit models. They can be applied to other latent variable models,
e.g. censored regression models like tobit models and panel or financial
time series data with discrete responses/missing entries. It is also
not limited to sparse covariance/precision matrix estimation. Any
estimation strategy that directly uses the latent response variables
for structured parameter estimation, e.g. penalized regression, quasi-maximum
likelihood, factor model-based estimation as in \cite{chamberlain1982arbitrage}
can be combined with the EM algorithm for latent variable models.%
\begin{comment}
 The key is the philosophy of dealing with identification problems
using model selection. Even if the structures are not sparse per se,
we may still perform model selection on the MLE problem by requiring,
for example, the covariance matrix to be low rank/have small trace
norm. Such regularizations help with the identification problem, and
if the regularization strength is not too large, the estimates will
be close to solutions to the original MLE. 
\end{comment}

Finally, there are several questions that are worth investigating
further. First, the number of Monte Carlo samples in each EM iteration
and its relation with convergence speed, and the reason why one or
a few Monte Carlo samples seem to suffice. Second, the effect of sparsity
regularization on reducing noise and number of Monte Carlo samples
required for convergence. Third, since our consistency results are
about particular local optima of the non-convex regularized MLE problem,
it is important to investigate whether the EM algorithm reaches such
a local optima. Empirical results suggest that indeed the correct
sparsity patterns are recovered by EM algorithm-based optimization
schemes. 
